Explaining Image Classifiers using Statistical Fault Localization

The black-box nature of deep neural networks (DNNs) makes it impossible to understand why a particular output is produced, creating demand for "Explainable AI". In this paper, we show that statistical fault localization (SFL) techniques from software engineering deliver high quality explanations of the outputs of DNNs, where we define an explanation as a minimal subset of features sufficient for making the same decision as for the original input. We present an algorithm and a tool called DeepCover, which synthesizes a ranking of the features of the inputs using SFL and constructs explanations for the decisions of the DNN based on this ranking. We compare explanations produced by DeepCover with those of the state-of-the-art tools GradCAM, LIME, SHAP, RISE and Extremal and show that explanations generated by DeepCover are consistently better across a broad set of experiments. On a benchmark set with known ground truth, DeepCover achieves 76.7% accuracy, which is 6% better than the second best Extremal.

==> exp.tex <==
\definecolor{Gray}{gray}{0.9}
\definecolor{LightCyan}{rgb}{0.88,1,1}
\newcolumntype{g}{>{\columncolor{Gray}}r}


\section{Experiments}
\label{sec:experiments}

We conduct experiments using the well-known MNIST {Handwritten Image Dataset}~\cite{MNIST},
the CIFAR-10 dataset~\cite{krizhevsky2009learning} on small images,
and the ImageNet benchmark~\cite{imagenet} from the large-scale visual recognition challenge.  
For clarity, our experiments are classified into four classes: \emph{\ding{192}~bug finding
\ding{193}~DNN safety statistics \ding{194}~testing efficiency \ding{195}~DNN internal structure
analysis}, and results will be labeled correspondingly. We also explain the relation
between our criteria and the existing ones.
All implementations, and the data discussed in this section, are available
online\footnote{Anonymously available from dropbox link \url{https://goo.gl/SMDJXH}}.

In our implementation, %every time the $get\_input\_pair$ is called we
%randomly select 40 correctly labeled inputs to construct the $data\_set$. 
the objective $\min{\distance{x_2\!-\!x_1}{\infty}}$ is used in all LP
calls, to find good adversarial examples with respect to the test
coverage conditions.  Moreover, we use 
$\valuefunction = \frac{u_{k+1,j}[x_2]}{u_{k+1,j}[x_1]}\geq \sigma$
%
%\begin{equation}
%\valuefunction = \frac{u_{k+1,j}[x_2]}{u_{k+1,j}[x_1]}\geq \sigma
%\end{equation} 
%
with $\sigma=2$ for $g$ in $SV^g$ and $\sigma=5$ for
$VV^{\valuefunction_1, \valuefunction_2}$ (with respect to $\valuefunction_2$).  
We admit that such choices are experimental. For generality and to
speed up the experiments, we leave the value function $\valuefunction_1$ unspecified. 
Providing a specific $\valuefunction_1$ may require more effort to find an
$x_2$ (because $\valuefunction_1$ is an additional constraint), but the
resulting $x_2$ can be better.
%with respect to $\valuefunction_1$.




%\begin{table*}
%    \def\arraystretch{1.2}
%    \scalebox{0.65}{
%    \begin{tabular}{|c|c|rg|rg|rg|rg|rg|} \hline
%      & hidden layers & $M_{\covered{SS}{}{}}$ & $AE_{\covered{SS}{}{}}$ &  $M_{\covered{VS}{\valuefunction}{}}$ & $AE_{\covered{VS}{\valuefunction}{}}$ &  $M_{\covered{SV}{g}{}}$ & $AE_{\covered{SV}{g}{}}$ &  $M_{\covered{VV}{\valuefunction_1,\valuefunction_2}{}}$ & $AE_{\covered{VV}{\valuefunction_1, \valuefunction_2}{}}$ \\\hline
%      $\networks_1$ & 67x22x63       & 99.7\% & 18.9\% & 100\% & 15.8\% & 100\% &6.7\% & 100\% & 21.1\%  \\\hline
%      $\networks_2$ & 59x94x56x45    & 98.5\% &  9.5\% & 100\% & 6.8\% & 99.9\% & 3.7\% & 100\% & 11.2\% \\\hline
%      $\networks_3$ & 72x61x70x77    & 99.4\% &  7.1\% & 100\% & 5.0\% & 99.9\% & 3.7\% & 98.6\% & 11.0\%     \\\hline
%      $\networks_4$ & 65x99x87x23x31 & 98.4\% &  7.1\% & 100\% & 7.2\% & 99.8\% & 3.7\% & 98.4\% & 11.2\%  \\\hline
%      $\networks_5$ & 49x61x90x21x48 & 89.1\% & 11.4\% & 99.1\%& 9.6\%& 99.4\%& 4.9\%& 98.7\%& 9.1\% \\\hline
%      $\networks_6$ & 97x83x32       &100.0\% &  9.4\% & 100\%& 5.6\%& 100\%& 3.7\%& 100\%& 8.0\%  \\\hline
%      $\networks_7$ & 33x95x67x43x76 & 86.9\% &  8.8\% & 100\%& 7.2\%& 99.2\%& 3.8\%& 96\%& 12.0\% \\\hline
%      $\networks_8$ & 78x62x73x47    & 99.8\% &  8.4\% & 100\%& 9.4\%& 100\%& 4.0\%& 100\%& 7.3\% \\\hline
%      $\networks_9$ & 87x33x62       &100.0\% & 12.0\% & 100\%& 10.5\%& 100\%& 5.0\%& 100\%& 6.7\% \\\hline
%   $\networks_{10}$ & 76x55x74x98x75 & 86.7\% &  5.8\% & 100\%& 6.1\%& 98.3\%& 2.4\%& 93.9\%& 4.5\% \\\hline
%
%    \end{tabular}
%    }
%    \captionof{table}{Coverage results on 10 DNNs with different covering methods}
%    \label{tab:results}
%\end{table*}


\begin{figure*}[!htb]
\begin{minipage}[b]{0.55\textwidth}
    \def\arraystretch{1.2}
    \scalebox{0.7}{
    \begin{tabular}{|c|c|rg|rg|rg|rg|rg|} \hline
      & hidden layers & $M_{\covered{SS}{}{}}$ & $AE_{\covered{SS}{}{}}$ &  $M_{\covered{VS}{\valuefunction}{}}$ & $AE_{\covered{VS}{\valuefunction}{}}$ &  $M_{\covered{SV}{g}{}}$ & $AE_{\covered{SV}{g}{}}$ &  $M_{\covered{VV}{\valuefunction_1,\valuefunction_2}{}}$ & $AE_{\covered{VV}{\valuefunction_1, \valuefunction_2}{}}$ \\\hline
      $\networks_1$ & 67x22x63       & 99.7\% & 18.9\% & 100\% & 15.8\% & 100\% &6.7\% & 100\% & 21.1\%  \\\hline
      $\networks_2$ & 59x94x56x45    & 98.5\% &  9.5\% & 100\% & 6.8\% & 99.9\% & 3.7\% & 100\% & 11.2\% \\\hline
      $\networks_3$ & 72x61x70x77    & 99.4\% &  7.1\% & 100\% & 5.0\% & 99.9\% & 3.7\% & 98.6\% & 11.0\%     \\\hline
      $\networks_4$ & 65x99x87x23x31 & 98.4\% &  7.1\% & 100\% & 7.2\% & 99.8\% & 3.7\% & 98.4\% & 11.2\%  \\\hline
      $\networks_5$ & 49x61x90x21x48 & 89.1\% & 11.4\% & 99.1\%& 9.6\%& 99.4\%& 4.9\%& 98.7\%& 9.1\% \\\hline
      $\networks_6$ & 97x83x32       &100.0\% &  9.4\% & 100\%& 5.6\%& 100\%& 3.7\%& 100\%& 8.0\%  \\\hline
      $\networks_7$ & 33x95x67x43x76 & 86.9\% &  8.8\% & 100\%& 7.2\%& 99.2\%& 3.8\%& 96\%& 12.0\% \\\hline
      $\networks_8$ & 78x62x73x47    & 99.8\% &  8.4\% & 100\%& 9.4\%& 100\%& 4.0\%& 100\%& 7.3\% \\\hline
      $\networks_9$ & 87x33x62       &100.0\% & 12.0\% & 100\%& 10.5\%& 100\%& 5.0\%& 100\%& 6.7\% \\\hline
   $\networks_{10}$ & 76x55x74x98x75 & 86.7\% &  5.8\% & 100\%& 6.1\%& 98.3\%& 2.4\%& 93.9\%& 4.5\% \\\hline

    \end{tabular}
    }
    \captionof{table}{Coverage results on 10 DNNs with different covering methods}
    \label{tab:results}
\end{minipage} \hspace{0.5cm}
%\begin{minipage}[b]{0.275\textwidth}
%\centering
%\includegraphics[width=\linewidth]{images/ss-distance-map}
%\caption{Adversarial example curves}
%\label{fig:ss-distance-map}
%\end{minipage}
%\begin{minipage}[b]{0.3\textwidth}
%\centering
%\includegraphics[width=\linewidth]{images/ss-distance-map}
%\caption{Adversarial example curves}
%\label{fig:ss-distance-map}
%\end{minipage}
\begin{minipage}[b]{0.4\textwidth}
\centering
\begin{tabular}{cc}
  \subfloat[from 9 to 8 ($b=0.02$)]{
    \includegraphics[width=0.36\linewidth]{images/9-8-d002}
    \label{fig:ad1}
  }
  &
  \subfloat[from 8 to 2 ($b=0.05$)]{
    \includegraphics[width=0.36\linewidth]{images/8-2-d005}
    \label{fig:ad2}
  }
  \\
  \subfloat[from 1 to 7 ($b=0.1$)]{
    \includegraphics[width=0.36\linewidth]{images/1-7-d01}
    \label{fig:ad3}
  }
  &
  \subfloat[from 0 to 9 ($b=0.2$)]{
    \includegraphics[width=0.36\linewidth]{images/0-9-d02}
    \label{fig:ad4}
  }
\end{tabular}
%\caption{Adversarial examples: (a) $9\rightarrow 8$; (b)$8\rightarrow 2$; (c) $1\rightarrow 7$; (d) $0\rightarrow 9$}
%\caption{Adversarial examples}
\caption{Selected adversarial examples: $b$ measures the $L^{\infty}$-norm distance between the two inputs} 
\label{fig:ads}
\end{minipage}
\end{figure*}


%\begin{minipage}[b]{0.275\textwidth}
%\centering
%\includegraphics[width=\linewidth]{images/ss-distance-map}
%\caption{Adversarial example curves}
%\label{fig:ss-distance-map}
%\end{minipage}

\begin{figure}[!htb]
\centering
\includegraphics[width=0.55\columnwidth]{images/ss-distance-map}
\caption{Adversarial example curves that record the accumulated percentage of
adversarial examples that fall into each distance:
the adversarial distance measures the distance between an adversarial example and the original input}
\label{fig:ss-distance-map}
\end{figure}

%\begin{figure}[!htb]
%\centering
%    \scalebox{0.65}{
%\begin{tabular}{cc}
%  \subfloat[from 9 to 8 ($b=0.02$)]{
%    \includegraphics[width=0.36\linewidth]{images/9-8-d002}
%    \label{fig:ad1}
%  }
%  &
%  \subfloat[from 8 to 2 ($b=0.05$)]{
%    \includegraphics[width=0.36\linewidth]{images/8-2-d005}
%    \label{fig:ad2}
%  }
%  \\
%  \subfloat[from 1 to 7 ($b=0.1$)]{
%    \includegraphics[width=0.36\linewidth]{images/1-7-d01}
%    \label{fig:ad3}
%  }
%  &
%  \subfloat[from 0 to 9 ($b=0.2$)]{
%    \includegraphics[width=0.36\linewidth]{images/0-9-d02}
%    \label{fig:ad4}
%  }
%\end{tabular}
%}
%\caption{Selected adversarial examples: $b$ measures the $L^{\infty}$-norm distance between the two inputs} %(a) $9\rightarrow 8$; (b)$8\rightarrow 2$; (c) $1\rightarrow 7$; (d) $0\rightarrow 9$}
%%\caption{Adversarial examples}
%\label{fig:ads}
%\end{figure}

%\begin{figure*}[!htb]
%\begin{minipage}[b]{0.3\textwidth}
%\centering
%\includegraphics[width=\linewidth]{images/ss-distance-map}
%\caption{Adversarial example curves}
%\label{fig:ss-distance-map}
%\end{minipage}
%\begin{minipage}[b]{0.3\textwidth}
%\centering
%\begin{tabular}{cc}
%  \subfloat[from 9 to 8 ($b=0.02$)]{
%    \includegraphics[width=0.36\linewidth]{images/9-8-d002}
%    \label{fig:ad1}
%  }
%  &
%  \subfloat[from 8 to 2 ($b=0.05$)]{
%    \includegraphics[width=0.36\linewidth]{images/8-2-d005}
%    \label{fig:ad2}
%  }
%  \\
%  \subfloat[from 1 to 7 ($b=0.1$)]{
%    \includegraphics[width=0.36\linewidth]{images/1-7-d01}
%    \label{fig:ad3}
%  }
%  &
%  \subfloat[from 0 to 9 ($b=0.2$)]{
%    \includegraphics[width=0.36\linewidth]{images/0-9-d02}
%    \label{fig:ad4}
%  }
%\end{tabular}
%%\caption{Adversarial examples: (a) $9\rightarrow 8$; (b)$8\rightarrow 2$; (c) $1\rightarrow 7$; (d) $0\rightarrow 9$}
%\caption{Adversarial examples}
%\label{fig:ads}
%\end{minipage}
%\end{figure*}

\begin{figure*}[!htb]
%\begin{minipage}[b]{0.25\textwidth}
%\centering
%\begin{tabular}{cc}
%  \subfloat[from 9 to 8 ($b=0.02$)]{
%    \includegraphics[width=0.36\linewidth]{images/9-8-d002}
%    \label{fig:ad1}
%  }
%  &
%  \subfloat[from 8 to 2 ($b=0.05$)]{
%    \includegraphics[width=0.36\linewidth]{images/8-2-d005}
%    \label{fig:ad2}
%  }
%  \\
%  \subfloat[from 1 to 7 ($b=0.1$)]{
%    \includegraphics[width=0.36\linewidth]{images/1-7-d01}
%    \label{fig:ad3}
%  }
%  &
%  \subfloat[from 0 to 9 ($b=0.2$)]{
%    \includegraphics[width=0.36\linewidth]{images/0-9-d02}
%    \label{fig:ad4}
%  }
%\end{tabular}
%%\caption{Adversarial examples: (a) $9\rightarrow 8$; (b)$8\rightarrow 2$; (c) $1\rightarrow 7$; (d) $0\rightarrow 9$}
%\caption{Adversarial examples}
%\label{fig:ads}
%\end{minipage}
%\begin{minipage}[b]{0.25\textwidth}
%\centering
%\includegraphics[width=\linewidth]{images/ss-distance-map}
%\caption{Adversarial curves}
%\label{fig:ss-distance-map}
%\end{minipage}
\begin{minipage}[b]{0.35\textwidth}
\centering
\includegraphics[width=0.75\linewidth]{images/ss-top10}
\caption{$\covered{SS}{}{}$ vs. $\covered{SS}{w10}{}$. Results demonstrate that
the SS coverage and its top-weight simplification have similar coverage levels ($M_{SS}-M_{SS^{w10}}$)
and percentages of adversarial examples ($AE_{SS}-AE_{SS^{w10}}$)}
\label{fig:ss-top10}
\end{minipage}\hspace{0.5cm}
\begin{minipage}[b]{0.6\textwidth}
\centering
\begin{tabular}{cc}
  %\subfloat[Layerwise coverage]{
  \subfloat[]{
    \includegraphics[width=0.45\linewidth]{images/layerwise-ss-coverage}
    \label{fig:scc-layerwise-coverage}
  }\hfill
  &
  %\subfloat[Adversarial example distribution]{
  \subfloat[]{
    \includegraphics[width=0.45\linewidth]{images/layerwise-ss-bugs}
    \label{fig:scc-layerwise-bugs}
  }
\end{tabular}
\caption{SS coverage by layer: (a) the coverage level per DNN layer; (b) the detected adversarial examples
at each layer with respect to the total amount of adversarial examples} 
\label{fig:ssc-layerwise}
\end{minipage}
\end{figure*}



\subsection{MNIST}

%We use the well-known MNIST \emph{Handwritten Image Dataset} to train a~set
%of 10 fully connected DNNs to perform classification.  Each DNN has an input
%layer of $28\times 28=784$ neurons and an output layer of $10$ neurons.  The
%number of hidden layers for each DNN is randomly sampled from the set of $\{3,
%4, 5\}$ and at each hidden layer, the number of neurons are uniformly
%selected from $20$ to $100$.  Every DNN is trained until an accuracy of at
%least $97.0\%$ is reached on the MNIST validation data.  Details on the
%structure of the DNNs are given in Table~\ref{tab:results}.
We randomly generate, and then train, a set of 10 fully connected DNNs, such that each network has an accuracy of at
least $97.0\%$ on the MNIST validation data. 
%
%We train a~set of 10 fully connected DNNs to perform classification.  
%The number of hidden layers for each DNN is randomly sampled from the set of
%$\{3, 4, 5\}$ and at each hidden layer, the number of neurons are uniformly
%selected from $20$ to $100$.  Every DNN is trained until an accuracy of at
%least $97.0\%$ is reached on the MNIST validation data.  
The detailed network structure, and the number of neurons per layer, are given in Table~\ref{tab:results}. Every DNN input has
been normalised into $[0,1]^{28\times 28}$.
Experiments were conducted on a MacBook Pro
(2.5\,GHz Intel Core i5, 8\,GB  memory).

\commentout{
\subsection{Hypothesis 1: Neuron coverage is Easy}

Neuron coverage is a simple test coverage metric proposed
in~\cite{PCYJ2017}.  It~was applied as one of the dual optimization
objectives to compute adversarial examples for DNNs.  Unfortunately, as a
test criterion, neuron coverage is inadequate.  In particular, a test
suite with high neuron coverage is not sufficient to increase confidence in
the neural network in safety-critical domains.

To demonstrate this, for each DNN tested, we randomly pick $25$ images from
the MNIST test dataset.  For each selected image, to maximize the neuron
coverage, if an input neuron is not activated (i.e., its activation value
is equal to 0), we sample its value from $[0, 0.1]$.  Then we measure
the neuron coverage of the DNN by using the generated test suite of $25$
images.  As a result, for all $10$ DNNs, we obtain almost 100\% neuron
coverage.  Our simple experiment here demonstrates that it is
straight-forward to obtain a trivial test suite that has high neuron
coverage but does not provide any adversarial examples.

As stated in~\cite{ZHM1997}, the role of test adequacy is a contributory
factor in building confidence in the repeated cycle of testing, debugging,
modifying program, and then testing again.  The above experimental result
shows that neuron coverage does not serve well in this role.

\subsection{Hypothesis 2: Random Testing is Inefficient}
\label{sec:random}

Previous research~\cite{ZHM1997} has observed that, while easy to perform,
random testing does not yield high confidence in software reliability, or
more formally, test adequacy is typically low.
%
%More precisely, it is believed \cite{} that random testing can be useful for execution errors such as memory leakage, but is less effective in program logic errors. The requirement for the DNNs can be reasonably seen as program logic error. 
%
Our experiments confirm this for the specific case of DNNs.

For each DNN, we first choose an image from the MNIST test dataset, denoted
by~$x$.  Subsequently, we randomly sample $10^5$ inputs in the region
bounded by $x\pm 0.1$, and we check whether an adversarial example exists
for the original image $x$.  Using this process, we have obtained
adversarial examples for only a single one of the $10$ DNNs; for the other
nine DNNs, we did not observe any adversarial examples among the $10^5$
randomly generated images.

More importantly, random testing does not provide information on the
adequacy level achieved.  Though it can be used to generate test cases for
simple criteria such as neuron coverage, it is not trivial to apply random
testing for complex metrics, such as the ones given in this paper, which
require independent sign change or value change of particular neuron
combinations.\footnote{However, we have no intention to discourage the use of
dynamic testing for DNNs, which has been under-investigated.  On the
contrary, we tend to expect that a more carefully designed dynamic testing method,
together with white-box techniques like algorithms in our paper, can improve
the performance and efficiency for testing DNNs.}
}
%\subsection{SS, SV, DS, and DV Cover}


We apply the  covering method defined in Section~\ref{sec:criteria}. %,
%for the SS, SV, VS, and VV covering
%methods.  
Besides the coverage $M_f$,
%for each method, 
we also measure the
percentage of adversarial examples among all test pairs in the test suite,
denoted by $AE_f$. % with
%$f\in\{\covered{SS}{}{},\covered{VS}{\valuefunction}{},\covered{SV}{\valuefunction}{},\covered{VV}{\valuefunction_1,\valuefunction_2}{}\}$.
%
%For testing each neuron pair, our algorithms randomly select a test data set of 40 images from MNIST test data set.
%
%We further investigate the use of the ``top 10 weights'' simplification of
%SS coverage ($\covered{SS}{w10}{}$). %, results of which are represented by $M_{\covered{SS}{w10}{}}$ and $AE_{\covered{SS}{w10}{}}$. 
\emph{Thanks to the use of LP optimisation, the feature in this part
is fine-grained to single neuron level.} That is, each feature pair 
is in fact a neuron pair.




\paragraph{DNN Bug finding \ding{192}}

%The full testing results are reported in Table~\ref{tab:results}.
The 
%full 
testing results, as reported in Table \ref{tab:results}, are promising:
(1) the test case generation algorithm
%are 
effectively %, as they %are able to 
achieves high coverage for all covering criteria,
and (2) the covering methods 
%designed 
are considered useful, supported by the fact that a significant
portion of adversarial examples are identified. %It is worthy of mentioning that, 
We note that, for neuron coverage \cite{PCYJ2017}, 
%we can easily achieve
a high coverage can be easily achieved by selecting a few non-adversarial test cases, which we generate.




\commentout{
\begin{table*}[!htb]
  \begin{center}
    \def\arraystretch{1.2}    
\scalebox{0.7}{
    \begin{tabular}{|c|c|rg|rg|rg|rg|rg|} \hline
      & hidden layers & $M_{\covered{SS}}$ & $AE_{\covered{SS}}$ &  $M_{\covered{VS}^{\valuefunction}}$ & $AE_{\covered{VS}^{\valuefunction}}$ &  $M_{\covered{SV}^g}$ & $AE_{\covered{SV}^g}$ &  $M_{\covered{DV}^{\distancefunction,g}}$ & $AE_{\covered{VV}^{\valuefunction_1, \valuefunction_2}}$ \\\hline
      $\networks_1$ & 67x22x63       & 99.7\% & 18.9\% & 100\% & 15.8\% & 100\% &6.7\% & 100\% & 21.1\%  \\\hline
      $\networks_2$ & 59x94x56x45    & 98.5\% &  9.5\% & 100\% & 6.8\% & 99.9\% & 3.7\% & 100\% & 11.2\% \\\hline
      $\networks_3$ & 72x61x70x77    & 99.4\% &  7.1\% & 100\% & 5.0\% & 99.9\% & 3.7\% & 98.6\% & 11.0\%     \\\hline
      $\networks_4$ & 65x99x87x23x31 & 98.4\% &  7.1\% & 100\% & 7.2\% & 99.8\% & 3.7\% & 98.4\% & 11.2\%  \\\hline
      $\networks_5$ & 49x61x90x21x48 & 89.1\% & 11.4\% & 99.1\%& 9.6\%& 99.4\%& 4.9\%& 98.7\%& 9.1\% \\\hline
      $\networks_6$ & 97x83x32       &100.0\% &  9.4\% & 100\%& 5.6\%& 100\%& 3.7\%& 100\%& 8.0\%  \\\hline
      $\networks_7$ & 33x95x67x43x76 & 86.9\% &  8.8\% & 100\%& 7.2\%& 99.2\%& 3.8\%& 96\%& 12.0\% \\\hline
      $\networks_8$ & 78x62x73x47    & 99.8\% &  8.4\% & 100\%& 9.4\%& 100\%& 4.0\%& 100\%& 7.3\% \\\hline
      $\networks_9$ & 87x33x62       &100.0\% & 12.0\% & 100\%& 10.5\%& 100\%& 5.0\%& 100\%& 6.7\% \\\hline
   $\networks_{10}$ & 76x55x74x98x75 & 86.7\% &  5.8\% & 100\%& 6.1\%& 98.3\%& 2.4\%& 93.9\%& 4.5\% \\\hline
    \end{tabular}
}
  \end{center}
  \caption{Results on 10 DNNs with the SS, VS, SV and VV covering methods}
  \label{tab:results}
\end{table*}


\begin{table}[]
\centering
\def\arraystretch{1.2}    
\scalebox{0.8}{
  \begin{tabular}{|c|c|r|rc|r|r|r|} \hline
  \multirow{2}{*}{} & \multirow{2}{*}{$\sum_{1<k\leq K}s_k$} &  \multirow{2}{*}{$|\neuronpairs(\networks)|$} & \multicolumn{5}{c|}{$|\testsuites|$}\\\cline{4-8}
                    & & & $\covered{SS}$ &  $(\covered{SS}^{w10})$  & $\covered{DS}^{\distancefunction}$ & $\covered{SV}^g$  & $\covered{DV}^{\distancefunction,g}$ \\ \hline
    $\networks_1$ & 162 & 3490 & 3478& (949)& 95 & 3490& 95\\\hline
    $\networks_{2}$ & 264 & 13780& 13569& (2037)& 205& 13779& 205\\\hline
    $\networks_{3}$ & 290 & 14822& 14739 & (2170)& 218& 14820& 215\\\hline
    $\networks_{4}$ & 315 & 18072& 17779 & (2409)& 250& 18028& 246\\\hline
    $\networks_{5}$ & 279 & 11857& 10567& (2120)& 228& 11780& 227\\\hline
    $\networks_{6}$ & 222 & 11027& 11027& (1250)& 125& 11027& 125\\\hline
    $\networks_{7}$ & 324 & 16409& 14264& (2593)& 291& 16275& 280\\\hline
    $\networks_{8}$ & 270 & 13263& 13235& (1917)& 192& 13263& 192\\\hline
    $\networks_{9}$ & 192 & 5537& 5537 & (1050)& 105& 5537& 105\\\hline
    $\networks_{10}$ & 388 & 23602& 20459& (2806)& 312& 23203& 293\\\hline
  \end{tabular}
}
\caption{Test suites generated using different criteria}
\label{tab:tests}
\end{table}
}


\paragraph{DNN safety analysis \ding{193}}

The coverage $M_f$ and adversarial example percentage $AE_f$ together provide
quantitative statistics to evaluate a DNN.  Generally speaking, given a test suite, a DNN with
a high 
$M_f$
, and a low 
$AE_f$
is considered 
robust.  
In addition, we can
study the \emph{adversarial quality}
%
%Because our test generation minimizes the distance when computing new
%input pairs (from which adversarial examples are distinguished), 
%To evaluate 
%the quality of obtained adversarial examples
%, called \emph{adversarial quality}, 
by 
%can 
plotting a distance curve
to see how close the adversarial example is to the correct input.  %Let us
%take a further look at 
Take a closer look into the results of SS coverage for the last three DNNs in
Table~\ref{tab:results}.  As illustrated in Figure~\ref{fig:ss-distance-map},
the horizontal axis measures the $L^{\infty}$
distance and the vertical axis reports the accumulated percentage of
adversarial examples that fall into this distance.  A~more robust DNN will have
its shape in the small distance end (towards~0) lower, as the reported
adversarial examples are relatively farther from their original correct
inputs.  Intuitively, this means that more effort needs to be made %in order
to fool a robust DNN from correct classification into mislabelling.
Figure~\ref{fig:ads} exhibits several adversarial examples found during the testing
with different distances.  The value of $b$ is 
%used 
to indicate the
closeness, and instantiate the safety property we define in Section~\ref{sec:safety}.
\commentout{
\begin{figure}[!htb]
\centering
\includegraphics[width=0.6\columnwidth]{images/ss-distance-map}
\caption{SS coverage distance curves of 3 DNNs}
\label{fig:ss-distance-map}
\end{figure}

\commentout{
\begin{figure}[!htb]
\captionsetup{justification=centering}
\centering
\begin{tabular}{cc}
	
  \subfloat[$9$ to $8$ with $b=0.02$]{
    \includegraphics[width=0.30\columnwidth]{images/9-8-d002}
    \label{fig:ad1}
  }
  &
  \subfloat[$8$ to $2$ with $b=0.05$]{
    \includegraphics[width=0.30\columnwidth]{images/8-2-d005}
    \label{fig:ad2}
  }
  \\
  \subfloat[$1$ to $7$ with $b=0.1$]{
    \includegraphics[width=0.30\columnwidth]{images/1-7-d01}
    \label{fig:ad3}
  }
  &
  \subfloat[$0$ to $9$ with $b=0.2$]{
    \includegraphics[width=0.30\columnwidth]{images/0-9-d02}
    \label{fig:ad4}
  }
\end{tabular}
\caption{Examples of adversarial examples}
\label{fig:ads}
\end{figure}
}

\begin{figure}[!htb]
\centering
\includegraphics[width=0.6\columnwidth]{images/ss-top10}
\caption{SS coverage vs SS coverage with top 10 weights}
\label{fig:ss-top10}
\end{figure}
}

\paragraph{SS coverage with top weights \ding{194}}

For SS coverage criteria with neuron pairs, 
%the covering method with sign change of condition features, 
there are
totally $|O|$ test requirements for $O\subseteq \neuronpairs(\networks)$. 
We note that $|\neuronpairs(\networks)|= \sum_{k=2}^{K} s_k \cdot s_{k-1}$. 
To reduce the test suite size, we define 
%an
%alternative definition of $\neuronpairs(\networks)$ 
$O$ as follows: 
$(\feature_{k,i},\feature_{k+1,j})\in O$ only when
the weight is one of the $\kappa$ largest among $\{|w_{k,i',j}|~|~i'\in
[1\dots s_{k}]\}$. The rationale is that condition neurons do not
equally affect their decision, and those with higher (absolute) weights are
likely to have a larger influence. 

Figure~\ref{fig:ss-top10} shows the difference, on coverage and adversarial example 
percentages, between SS coverage and its simplification with $\kappa=10$, denoted by $SS^{w10}$.  
%for the testing of 10 DNNs.  
In general, the two are comparable.  This is very
useful in practice, as the ``top weights'' simplification mitigates the size of the rsulting test suite, and it is thus able to behave as a faster pre-processing phase and
even provide an alternative with comparable results for SS coverage.

\commentout{
\begin{figure}[!htb]
\captionsetup{justification=centering}
\centering
\begin{tabular}{cc}
	
  \subfloat[Layerwise coverage]{
    \includegraphics[width=0.46\columnwidth]{images/layerwise-ss-coverage}
    \label{fig:scc-layerwise-coverage}
  }\hfill
  &
  \subfloat[Layerwise adversarial examples]{
    \includegraphics[width=0.46\columnwidth]{images/layerwise-ss-bugs}
    \label{fig:scc-layerwise-bugs}
  }
\end{tabular}
\caption{SS coverage by layers} 
\label{fig:ssc-layerwise}
\end{figure}
}

\paragraph{Layerwise behavior \ding{195}}

Our experiments show that different
layers of a DNN exhibit different behaviors in testing. 
Figure~\ref{fig:ssc-layerwise} reports the SS coverage results, collected in
adjacent layers.  In particular, Figure~\ref{fig:scc-layerwise-coverage}
gives the percentage of covered neuron pairs within individual adjacent
layers.  As we can see, when going deeper into the DNN, it can become harder
to cover of neuron pairs.  Under such circumstances, to improve the
coverage performance, the use of larger a $data\_set$ is needed when generating test
pairs.  Figure~\ref{fig:scc-layerwise-bugs} gives the percentage
of adversarial examples found at different layers (among the overall adversarial examples).  Interestingly, it seems
that most adversarial examples are found when testing the middle layers.
%of all DNNs
%tested.

\begin{table}
\centering
%\def\arraystretch{1.2}    
%\setlength\extrarowheight{5pt}
\scalebox{0.85}{
  \begin{tabular}{|l|ccc|ccc|ccc|} \hline
    \multirow{2}{*}{         } & \multicolumn{3}{c|}{$\networks_8$} &  \multicolumn{3}{c|}{$\networks_9$} & \multicolumn{3}{c|}{$\networks_{10}$}\\\cline{2-10}
                             & \#vars & $|\constraints|$ & $t$ & \#vars & $|\constraints|$ & $t$ & \#vars & $|\constraints|$ & $t$ \\\hline
    $L2\textnormal{-}3$             & 864 & 3294 & 0.58 & 873 & 3312 & 0.57 & 862 & 3290 & 0.49 \\
    $L3\textnormal{-}4$             & 926 & 3418 & 0.84 & 906 & 3378 & 0.61 & 917 & 3400 & 0.71 \\
    $L4\textnormal{-}5$             & 999 & 3564 & 0.87 & 968 & 3502 & 0.86 & 991 & 3548 & 0.75 \\
    $L5\textnormal{-}6$             & 1046& 3658 & 0.91 & --& --   &  --    & 1089& 3744 & 0.82 \\
    $L6\textnormal{-}7$             & -- & -- & -- & -- & -- & -- & 1164 & 3894 & 0.94 \\ 
    \hline
  \end{tabular}
}
\caption{Number of variables and constraints, and time cost of each LP call in test generation}
\label{tab:lp-call}
\end{table}

\paragraph{Cost of LP call \ding{194}}

Since LP encoding of the DNN (partial) activation pattern plays a key role
in the test generation, in this part we give details of the LP call cost,
even though LP is widely accepted as an efficient method. 
For every DNN, we select a set of neuron pairs, where each decision neuron
is at a different layer.  Then, we measure the number of variables and
constraints, and the time $t$ in seconds (averaged over 100
runs) spent on solving each LP call.  Results in Table
\ref{tab:lp-call} confirm that the LP model of a partial activation pattern
is indeed lightweight, and its complexity increases in a linear manner when
traversing into deeper layers of a DNN.



%\paragraph{Convolutional Neural Networks \ding{195}}
%
%%Criteria and testing techniques 
%
%%The testing approach in this paper can be generalized to 
%We conduct dedicated experiments for 
%convolutional
%neural networks (CNNs). 
%%
%%Without loss of generality, we skip the technical details
%%for defining a 
%CNN can be  treated as a special DNN such that the activation of a node in layer $k$
%is computed  by the activations of a subset of precedent nodes, 
% and each node belongs to a feature map in its layer. 
%%that is called the feature map.
%%The weights and bias that define a feature map are often said to be \emph{filters}.
%We trained two CNNs $\networks^c_1$ and $\networks^c_2$ with 14,208 and 1,536 hidden neurons, respectively, to validate the scalability of our approach.
%%
%%
%%In a CNN, a convolutional layer consists of
%%multiple \emph{feature maps}.  The weights and bias that define a feature
%%map are often said to be \emph{filters}.  Given a decision neuron inside
%%some feature map, its activation is computed by a subset of precedent
%%neurons that are processed by the associated filter.  
%%To investigate the
%%testing of CNNs, we trained two networks $\networks^c_1$ and
%%$\networks^c_2$, each having two convolutional layers followed by one fully
%%connected layer of 128 neurons.  $\networks^c_1$ (resp.~$\networks^c_2$) has
%%20 (resp.~2) filters for the first convolutional layer and 40 (resp.~4)
%%filters for the second convolutional layer.  The filters have size $5\times
%%5$ and every convolutional layer is augmented with a so-called max-pooling
%%layer of size $2\times 2$.  Overall, $\networks^c_1$ has 14208 hidden
%%neurons and $\networks^c_2$ is much smaller with 1536 hidden neurons.  This
%%is designed on purpose to conduct our testing approaches with different
%%scalabilities.
%\begin{table}[!htb]
%  \begin{center}
%  \scalebox{0.8}{
%    %\def\arraystretch{1.5}    
%    \begin{tabular}{|c|rg|rg|} \hline
%      & $M_{\covered{SS}{}{}}^{(1,1), (2,1)}$ & $AE_{\covered{SS}{}{}}^{(1,1), (2,1)}$ & $M_{\covered{SS}{}{}}^{(1,1), (2,2)}$ & $AE_{\covered{SS}{}{}}^{(1,1), (2,2)}$\\\hline
%       $\networks^c_1$ & 99.7\%& 1.6\%& 99.7\%& 1.5\%\\\hline
%       $\networks^c_2$ & 100\%& 7.6\%& 100\%& 6.8\%\\\hline
%    \end{tabular}
%  }
%  \end{center}
%  \caption{
%  %Feature map wise 
%  SS coverage results for CNNs}
%  \label{tab:cnn-results}
%\end{table}
%\bigskip
% This experiment is to understand the convolutional structures  through testing. % and results of SS coverage are analysed at feature map level. % that is, feature pairs from two specified feature maps are tested.  
%%
%%We use $f_{k,i}$ to denote the $i$-th feature map in the $k$-th
%%convolutional layer, and $M_{\covered{SS}{}{}}^{f_{k,i}}_{f_{k+1,j}}$ represents the
%%SS coverage among neuron pairs such that the condition neuron and decision
%%neuron are from $f_{k,i}$ and $f_{k+1,j}$ respectively.  Correspondingly,
%%$AE_{\covered{SS}{}{}}^{f_{k,i}}_{f_{i+1,j}}$ is for the adversarial percentage. 
%Results in Table \ref{tab:cnn-results} show the detailed testing information
%on several feature maps. % of the two CNNs.  
%The $M_{\covered{SS}{}{}}^{(k,i),(k+1,j)}$ is for the coverage when testing features between the $i$-th and the $j$-th feature map in layer $k$ and $k+1$, respectively,
%and $AE_{\covered{SS}{}{}}^{(k,i),(k+1,j)}$ is the corresponding adversarial example percentage.
%The use of more complex convolutional structures is
%justified through our testing, as a much smaller number of adversarial examples
%were found for $\networks^c_1$.
%\commentout{
%\begin{table}[!htb]
%  \begin{center}
%  \scalebox{0.8}{
%    %\def\arraystretch{1.5}    
%    \begin{tabular}{|c|rg|rg|} \hline
%      & $M_{\covered{SS}{}{}}^{f_{1,1}}_{f_{2,1}}$ & $AE_{\covered{SS}{}{}}^{f_{1,1}}_{f_{2,1}}$ & $M_{\covered{SS}{}{}}^{f_{1,1}}_{f_{2,2}}$ & $AE_{\covered{SS}{}{}}^{f_{1,1}}_{f_{2,2}}$\\\hline
%       $\networks^c_1$ & 99.7\%& 1.6\%& 99.7\%& 1.5\%\\\hline
%       $\networks^c_2$ & 100\%& 7.6\%& 100\%& 6.8\%\\\hline
%    \end{tabular}
%  }
%  \end{center}
%  \caption{Feature map wise SS coverage results}
%  \label{tab:cnn-results}
%\end{table}
%}

\subsection{CIFAR-10}

The CIFAR-10 dataset is a collection of 32x32 color images in 10 kinds of objects. Different from the MNIST case,
we need to train a DNN with convolutional layers in order to handle the CIFAR-10 image classification problem.
Without loss of generality, the activation of a node in the convolutional layer %$k$
is computed  by the activations of a subset of precedent nodes, and each node belongs to a \emph{feature map} in its layer. 
We apply the test case generation in Algorithm \ref{algo:aac-get-input-pair-search} for the SS coverage and  measure
the coverage results individually for decision features at each different layer. Overall, an SS coverage higher than 90\% is achieved
with a significant portion of adversarial examples.  
An interesting observation is as in Figure \ref{fig:cifar-adv-distribution} (\ding{195}), 
which shows that in this case
the causal changes of features at deeper layers are able to detect smaller perturbations of inputs that cause adversarial behaviours,
and this is likely to provide helpful feedback for developers to debug or tune the neural network parameters.
Selected adversarial examples are given in Figure \ref{fig:cifar-advs}. 

%\begin{figure}[!htb]
%\centering
%\includegraphics[width=0.55\columnwidth]{images/coverage-crop-tmp}
%\caption{{\color{red}**To be replaced by final results**}The average coverage result for feaure maps at different layers}
%\label{fig:cifar-coverage}
%\end{figure}

\begin{figure}[!htb]
\centering
\includegraphics[width=0.55\columnwidth]{images/cifar-errorbar-crop}
\caption{The averaged adversarial distance for decision features at different layers}
\label{fig:cifar-adv-distribution}
\end{figure}

\begin{figure}[!htb]
\captionsetup{justification=centering}
\centering
\begin{tabular}{cc}
  \subfloat[bird$\rightarrow$airplane]{
    \includegraphics[width=0.175\columnwidth]{images/examples/2092-original-2}
    \includegraphics[width=0.175\columnwidth]{images/examples/2092-adv-0}
    \label{fig:ad3}
  }
  &
  \subfloat[airplane$\rightarrow$cat]{
    \includegraphics[width=0.175\columnwidth]{images/examples/2606-original-0}
    \includegraphics[width=0.175\columnwidth]{images/examples/2606-adv-3}
    \label{fig:ad4}
  }
  %\\
  %\subfloat[bird$\rightarrow$cat]{
  %  \includegraphics[width=0.15\columnwidth]{images/examples/36-original-2}
  %  \includegraphics[width=0.15\columnwidth]{images/examples/36-adv-3}
  %  \label{fig:ad1}
  %}
  %&
  %\subfloat[deer$\rightarrow$frog]{
  %  \includegraphics[width=0.15\columnwidth]{images/examples/48-original-4}
  %  \includegraphics[width=0.15\columnwidth]{images/examples/48-adv-6}
  %  \label{fig:ad2}
  %}
\end{tabular}
\caption{Selected adversarial examples for CIFAR-10}
\label{fig:cifar-advs}
\end{figure}

%\vspace{-0.5cm}
\subsection{ImageNet}

We applied our methods to VGG16~\cite{vgg16}, a large-scale DNN trained on the ImageNet dataset. 
%The pre-trained
% in Keras~\cite{keras} is tested. 
 %In particular, the 
 The heuristic search algorithm~\ref{algo:aac-get-input-pair-search} is called to generate test cases. 
 %Still, we 
 We consider each
decision feature as a single set. 
The feature selection problem in machine learning is, by itself, an interesting topic and out of
the scope of this paper. Instead, 
to apply our covering method, we select arbitrary condition
features that are within certain sizes. In particular, a size parameter $\omega$ is defined for the
experiments such that a feature $\feature_{k,i}$ is required to have its size $\leq\omega\cdot s_k$. Recall that 
 $s_k$ is the number of neurons in layer $k$.

\paragraph{Different feature sizes~\ding{192}~\ding{193}~\ding{195}}
We apply SS coverage on 2,000 randomly sampled feature pairs %in the VGG16 model 
with 
$\omega\in\{0.1\%, 0.5\%, 1.0\%\}$. The covering method shows its effectiveness by returning
a test suite in which  $10.5\%$, $13.6\%$ and $14.6\%$ are
adversarial examples. %More interestingly, 
We report the adversarial examples' average distance and standard deviation
in Figure~\ref{fig:ssc-errorbar}.  The results confirm that there is a
relation between the feature pairs and the input perturbation.  Among the
generated adversarial examples, a more fine-grained feature is able to
capture smaller perturbations
%, which cause the adversarial examples, 
than a coarse one.

%\vspace{-0.4cm}
\begin{figure}[!htb]
\centering
\includegraphics[width=0.55\columnwidth]{images/ssc-errorbar}
%\includegraphics[width=0.5\columnwidth]{images/svc-curve}
\caption{Adversarial distance with different feature sizes: a smaller distance corresponds to more subtle
adversarial examples}
%; (right) Adversary curve for SV with neuron boundary}
\label{fig:ssc-errorbar}
\end{figure}
\vspace{0.4cm}

Results in Figure~\ref{fig:ssc-errorbar} are measured with $L^{\infty}$-norm that 
corresponds to the maximum changes %happen 
to a pixel. We observed that, though the change of each pixel is very small, for every adversarial example
a large portion (around $50\%$) of pixels are changed. A typical adversarial example image 
is given in Figure~\ref{fig:adv-traffic-light}. Overall, the detected adversarial examples are considered of high quality.

%\vspace{-0.25cm}
\begin{figure}[!htb]
\centering
\includegraphics[width=\columnwidth]{images/adv-trafficlight}
\caption{An adversarial example (``lipstick'') for the original traffic light input, with $L^{\infty}$ distance $0.26$.}
\label{fig:adv-traffic-light}
\end{figure}

\paragraph{SV with neuron boundary coverage~\ding{192}~\ding{193}}
\vspace{-0.35cm}
As shown in Section \ref{sec:comparison}, our covering methods are stronger than
neuron boundary coverage. In fact, neuron boundary is a special case of SV coverage,
%in this paper, 
when the value function %$g$ 
of the decision feature is designed to make
the activation exceed the specified boundary value. Similarly to the experiments
above, we generate a test suite using SV with neuron boundary coverage. We noticed that
accessing boundary activation values is likely to request bigger changes to be made in DNNs.
We set the feature size using $\omega=10\%$ and obtain a test suite with
$22.7\%$ adversarial examples. %However, if we look into the adversary quality, as shown
%in Figure~\ref{fig:ssc-errorbar}(right), 
However, the distance of these adversarial examples, with average $L^{\infty}$-norm distance 3.49 and standard deviation 3.88, is much greater than those for SS coverage.
\commentout{
\begin{figure}[!htb]
\centering
\includegraphics[width=0.5\columnwidth]{images/svc-curve}
\caption{The adversarial example curve when using SV with neuron boundary coverage}
\label{fig:sv-curve}
\end{figure}
}


==> experiments.tex <==
\section{Experimental Results}
\label{sec:experiments}

We implement the proposed method in Section \ref{sec:proposed} into the DeepCover framework for
testing deep learning software.
All experiments are conducted on a laptop with Intel i7-7820HQ (8) @ 3.900GHz, 16 GB memory and
Nvidia Quadro Graphics.

Images are still nowadays most important inputs for DNNs, and in this work we consider a variety of
popular image data sets, including

\begin{itemize}
\item MNIST~\cite{lecun1998gradient}: a database of 28x28 grayscale images for handwritten digits from 0 to 9,
\item CIFAR-10~\cite{krizhevsky2009learning}: a set of  32x32 colour images in 10 classes such as `horse' and `car',
\item ImageNet~\cite{russakovsky2015imagenet}: the benchmark for large scale visual recognition challenge, and
\item COCO~\cite{lin2014microsoft}: a large scale image captioning dataset.
\end{itemize}

We trained two DNNs for MNIST and CIFAR-10 image recognition. The pre-trained VGG16
model for Keras~\cite{VGG16} is used for the ImageNet case. 
We used one open source tool~\cite{captioning-tool}, which implements the technique in \cite{xu2015show},
to generate captions for COCO image inputs. The image captioning model consists of two parts:
a convolutional neural network (that is ResNet~\cite{He2016DeepRL} in our experiments) to extract visual
features from the image, and a LSTM recurrent neural network to decode these features into a sentence.

Thanks to the lightweight of spectrum based measures, the interpretation of each test input can be
fine-grained to the pixel level. Particularly, for each test input image, we apply DeepCover and 
report its top $\gamma$ most important pixels, with $\gamma\in\{1\%, 2\%, 5\%, 10\%, 20\%\}$
for the DNN to make its decision on the output.

Experiments in this section will answer the following three questions.

\begin{itemize}
\item[Q1] Do the interpretation results benefit people to understand how DNN makes its decisions based on the test inputs?
\item[Q2] Do the interpretation results indeed reflect the decision making in the DNN?
\item[Q3] What about the comparison between DeepCover and other tools on explaining outputs from machine learning algorithms?
\end{itemize}


\subsection{Interpretation does help understand DNN's decision making}

Results are shown in Figure \ref{fig:mnist-cifar} and \ref{fig:captioning}.
%At first, we are going to demonstrate that the results by DeepCover indeed help users
%understand test inputs for a DNN. Examples are as in Figure %\ref{fig:mnist}\ref{fig:cifar}\ref{fig:captioning}.
%More examples will be added.

\begin{figure}[!htb]
\centering
  \subfloat[]{
    \includegraphics[width=0.15\columnwidth]{images/mnist-example2/origin-7}
  }
  \subfloat[]{
    \includegraphics[width=0.15\columnwidth]{images/mnist-example2/zoltar-17}
  }
  \subfloat[]{
    \includegraphics[width=0.15\columnwidth]{images/mnist-example2/zoltar-38}
  }
  \subfloat[]{
    \includegraphics[width=0.15\columnwidth]{images/mnist-example2/zoltar-80}
  }
  \subfloat[]{
    \includegraphics[width=0.15\columnwidth]{images/mnist-example2/zoltar-164}
  } \\
  \subfloat[]{
    \includegraphics[width=0.15\columnwidth]{images/mnist-example3/origin-2}
  }
  \subfloat[]{
    \includegraphics[width=0.15\columnwidth]{images/mnist-example3/zoltar-17}
  }
  \subfloat[]{
    \includegraphics[width=0.15\columnwidth]{images/mnist-example3/zoltar-38}
  }
  \subfloat[]{
    \includegraphics[width=0.15\columnwidth]{images/mnist-example3/zoltar-80}
  }
  \subfloat[]{
    \includegraphics[width=0.15\columnwidth]{images/mnist-example3/zoltar-164}
  } \\
  \subfloat[]{
    \includegraphics[width=0.15\columnwidth]{images/cifar10-example3/origin-7}
  }
  \subfloat[]{
    \includegraphics[width=0.15\columnwidth]{images/cifar10-example3/zoltar-70}
  }
  \subfloat[]{
    \includegraphics[width=0.15\columnwidth]{images/cifar10-example3/zoltar-160}
  }
  \subfloat[]{
    \includegraphics[width=0.15\columnwidth]{images/cifar10-example3/zoltar-310}
  }
  \subfloat[]{
    \includegraphics[width=0.15\columnwidth]{images/cifar10-example3/zoltar-640}
  } \\
  \subfloat[]{
    \includegraphics[width=0.15\columnwidth]{images/cifar10-example4/origin-1}
  }
  \subfloat[]{
    \includegraphics[width=0.15\columnwidth]{images/cifar10-example4/zoltar-70}
  }
  \subfloat[]{
    \includegraphics[width=0.15\columnwidth]{images/cifar10-example4/zoltar-160}
  }
  \subfloat[]{
    \includegraphics[width=0.15\columnwidth]{images/cifar10-example4/zoltar-310}
  }
  \subfloat[]{
    \includegraphics[width=0.15\columnwidth]{images/cifar10-example4/zoltar-640}
  } \\
\caption{Examples of MNIST and CIFAR-10 inputs (first column) and their top $\gamma$ important pixels with $\gamma \in\{2\%, 5\%, 10\%, 20\%\}$}
\label{fig:mnist-cifar}
\end{figure}


%\begin{figure}[!htb]
%\centering
%  \subfloat[]{
%    \includegraphics[width=0.175\columnwidth]{images/cifar-example1/origin-9}
%    %\label{fig:mnist1-a}
%  }
%  \subfloat[]{
%    \includegraphics[width=0.175\columnwidth]{images/cifar-example1/zoltar-70}
%    %\label{fig:mnist1-b}
%  }
%  \subfloat[]{
%    \includegraphics[width=0.175\columnwidth]{images/cifar-example1/zoltar-160}
%    %\label{fig:mnist1-c}
%  }
%  \subfloat[]{
%    \includegraphics[width=0.175\columnwidth]{images/cifar-example1/zoltar-310}
%    %\label{fig:mnist1-d}
%  }\\
%  \subfloat[]{
%    \includegraphics[width=0.175\columnwidth]{images/cifar-example2/origin-6}
%    %\label{fig:mnist1-a}
%  }
%  \subfloat[]{
%    \includegraphics[width=0.175\columnwidth]{images/cifar-example2/zoltar-70}
%    %\label{fig:mnist1-b}
%  }
%  \subfloat[]{
%    \includegraphics[width=0.175\columnwidth]{images/cifar-example2/zoltar-160}
%    %\label{fig:mnist1-c}
%  }
%  \subfloat[]{
%    \includegraphics[width=0.175\columnwidth]{images/cifar-example2/zoltar-310}
%    %\label{fig:mnist1-d}
%  }\\
%\caption{Examples on CIFAR-10 image detection:
%The first column are the original test inputs and the following columns
%are their top 2\%, top 5\% and top 10\% important pixels for the DNN
%predictions.}
%\label{fig:cifar}
%\end{figure}

%\begin{figure*}[!htb]
%  \centering
%  \subfloat[]{
%    \includegraphics[width=0.15\linewidth]{images/imagenet-example1/origin-407}
%  }\hspace{0.cm}
%  \subfloat[]{
%    \includegraphics[width=0.15\linewidth]{images/imagenet-example1/zoltar-3020}
%  }\hspace{0.cm}
%  \subfloat[]{
%    \includegraphics[width=0.15\linewidth]{images/imagenet-example1/zoltar-7535}
%  }\hspace{0.cm}
%  \subfloat[]{
%    \includegraphics[width=0.15\linewidth]{images/imagenet-example1/zoltar-15060}
%  }\\
%  \caption{Explanations on ImageNet test inputs:}
%  \label{fig:imagenet}
%\end{figure*}

\begin{figure*}[!htb]
  \centering
  %\subfloat[]{
  %  \includegraphics[width=0.225\linewidth]{images/captioning-example1/origin-True}
  %}\hspace{0.cm}
  %\subfloat[]{
  %  \includegraphics[width=0.225\linewidth]{images/captioning-example1/zoltar-3020}
  %}\hspace{0.cm}
  %\subfloat[]{
  %  \includegraphics[width=0.225\linewidth]{images/captioning-example1/zoltar-7535}
  %}\hspace{0.cm}
  %\subfloat[]{
  %  \includegraphics[width=0.225\linewidth]{images/captioning-example1/zoltar-15060}
  %}\\
  \subfloat[]{
    \includegraphics[width=0.1\linewidth]{images/captioning-example2/origin-True}
  }\hspace{0.cm}
  \subfloat[]{
    \includegraphics[width=0.1\linewidth]{images/captioning-example2/zoltar-1515}
  }\hspace{0.cm}    
  \subfloat[]{
    \includegraphics[width=0.1\linewidth]{images/captioning-example2/zoltar-3020}
  }\hspace{0.cm}
  \subfloat[]{
    \includegraphics[width=0.1\linewidth]{images/captioning-example2/zoltar-7535}
  }\hspace{0.cm}
  \subfloat[]{
    \includegraphics[width=0.1\linewidth]{images/captioning-example2/zoltar-15060}
  }
  \subfloat[]{
    \includegraphics[width=0.1\linewidth]{images/captioning-example2/zoltar-30110}
  }\\
  \subfloat[]{
    \includegraphics[width=0.1\linewidth]{images/captioning-example3/origin-True}
  }\hspace{0.cm}
  \subfloat[]{
    \includegraphics[width=0.1\linewidth]{images/captioning-example3/zoltar-1515}
  }\hspace{0.cm}
  \subfloat[]{
    \includegraphics[width=0.1\linewidth]{images/captioning-example3/zoltar-3020}
  }\hspace{0.cm}
  \subfloat[]{
    \includegraphics[width=0.1\linewidth]{images/captioning-example3/zoltar-7535}
  }\hspace{0.cm}
  \subfloat[]{
    \includegraphics[width=0.1\linewidth]{images/captioning-example3/zoltar-15060}
  }
  \subfloat[]{
    \includegraphics[width=0.1\linewidth]{images/captioning-example3/zoltar-30110}
  }\\
  \subfloat[]{
    \includegraphics[width=0.1\linewidth]{images/captioning-example4/origin-True}
  }\hspace{0.cm}
  \subfloat[]{
    \includegraphics[width=0.1\linewidth]{images/captioning-example4/zoltar-1515}
  }\hspace{0.cm}
  \subfloat[]{
    \includegraphics[width=0.1\linewidth]{images/captioning-example4/zoltar-3020}
  }\hspace{0.cm}
  \subfloat[]{
    \includegraphics[width=0.1\linewidth]{images/captioning-example4/zoltar-7535}
  }\hspace{0.cm}
  \subfloat[]{
    \includegraphics[width=0.1\linewidth]{images/captioning-example4/zoltar-15060}
  }
  \subfloat[]{
    \includegraphics[width=0.1\linewidth]{images/captioning-example4/zoltar-30110}
  }
  \caption{Examples of COCO image inputs (first column) and their top $\gamma$
  important pixels with $\gamma \in\{1\%, 2\%, 5\%, 10\%, 20\%\}$
%(a) the first prediction is "a cat that is sitting on a toilet"
%(b) the second prediction is "a man is flying a kite in the field"
%(b) the third prediction is "a man riding a boat in the water"
%(b) the fourth prediction is "an airplane is flying in the sky"
}
  \label{fig:captioning}
\end{figure*}


\subsection{Interpretation does reflect the DNN's decision making}
Results are shown in Figure \ref{fig:comparison-mnist-cifar}.

%We just demonstrated that the spectrum to prioritise different parts of a test input
%can help people understand the test suite. However, how do we know that the
%higher ranked pixels in the spectrum are indeed more important for the DNN model
%to make its decision? To answer this, we design the following experiment.

%$\mathcal{N}[t]$ is the prediction of test input $t$ by the DNN $\mathcal{N}$.
%
%$t[p]$ is the value of a pixel $p$ for the test input $t$
%
%\paragraph{Experiment setup}
%
%\begin{enumerate}
%\item Pick up a test input $t$, based on which the adversarial example $t'$ is found s.t.
%$close(t, t')$ and $\mathcal{N}[t]\neq\mathcal{N}[t']$.
%\item Starting from an empty set $\mathcal{C}$, following some ordering $\mathcal{R}$,
%we iteratively pick up a pixel s.t. $t[p]\neq t'[p]$ and we reset its value for $t'$
%s.t. $t'[p]:=t[p]$. Subsequently, a) if $\mathcal{N}[t]\neq\mathcal{N}[t']$, add $p$ into $\mathcal{C}$
%and continue Step (2), otherwise, goto (1). 
%\end{enumerate}
%We call the final $\mathcal{C}$ the critical set of pixels that make
% $t$ and $t'$ have different predictions.
%Given $t$ and $t'$, following different orderings of pixels, the resulted critical sets can
%be different. Intuitively, given two critical sets $\mathcal{C}_1$ and $\mathcal{C}_2$,
%if the size of $\mathcal{C}_1$ is smaller, it indicates that $\mathcal{C}_1$ is more likely
%to contain more important pixels that affect the DNN's decision on the test input $t$.
%
%It is out of the scope of this paper to find the optimal set of pixels that differentiate
%the prediction of two inputs $t$ and $t'$, which by itself is a challenging research problem.
%Even if we successfully localise the the influential parts of a test input, optimising
%the adversarial example generation is a totally different prroblem that requires dedicated
%research work.
%\emph{Thus, we only use the critical set as a metric to evaluate the relative 
%effectiveness between different measures for prioritising pixels of the test input.}
%
%The spectrum returned by DeepCover is in fact an ordering of pixels. 
%We run the experiment following the above setup and we apply DeepCover to generate 
%the pixel ordering $\mathcal{R}$. We record sizes of the final critical sets.
%
%DeepCover supports a number of statistical measures. According to the evaluation
%results in \cite{landsberg2015evaluation}, Ochiai, Wong II and Tarantula have the
%best performance for traditional software. We are going to compare them for the purpose
%of explaining test suites for DNNs. 
%
%Results are in Figure \ref{fig:comparison-cifar}. 'Best' represents the best result 
%among all measures \{Ochiai, Wong II, Tarantula, Zoltar\}. We also consider generating
%critical sets randomly.
%First of all, DeepCover indeed localises these important pixels of an image input, as
%the critical sets following the prioritised spectrum are overall much smaller than the
%randomly constructed.
%Furthermore, among all measures, Wong II is shown more effective than others, however,
%the dominance by the 'Best' also indicates different measures most likely complement
%each other.

%\begin{figure}[!htb]
%  \centering
%  \includegraphics[width=0.95\columnwidth]{images/mnist-comparison}
%  \caption{Comparison with different measures on MNIST data: the percentage of DNN decisions (vertical axis) that can be restored by parts of the original inputs (horizontal axis)}
%  \label{fig:comparison-mnist}
%\end{figure}

%\begin{figure}[!htb]
%  \centering
%  \includegraphics[width=0.95\columnwidth]{images/cifar-comparison}
%  \caption{Comparison with different measures on CIFAR-10 data
  %: the horizontal axis indicates
%the critical set size and the vertical axis indicates the accumulated
%critical sets with a smaller size
%}
%  \label{fig:comparison-cifar}
%\end{figure}

\begin{figure*}[!htb]
  \centering
  \subfloat[(a)]{
    \includegraphics[width=0.45\linewidth]{images/mnist-comparison}
  }\hspace{0.cm}
  \subfloat[(b)]{
    \includegraphics[width=0.45\linewidth]{images/cifar-comparison}
  }\hspace{0.cm}
  \caption{Comparison with different measures on MNIST data (in (a)) and CIFAR-10 data (in (b)): the percentage of DNN decisions (vertical axis) that can be restored by parts of the original inputs (horizontal axis) when pixels are ordered using different measures {\color{red} this figure will be updated}}
  \label{fig:comparison-mnist-cifar}
\end{figure*}


%\begin{figure}[!htb]
%\centering
%  \subfloat[]{
%    \includegraphics[width=0.175\columnwidth]{images/tarantula/origin-7}
%    %\label{fig:mnist1-}
%  }
%  \subfloat[]{
%    \includegraphics[width=0.175\columnwidth]{images/tarantula/tarantula-70}
%    %\label{fig:mnist1-b}
%  }
%  \subfloat[]{
%    \includegraphics[width=0.175\columnwidth]{images/tarantula/tarantula-160}
%    %\label{fig:mnist1-c}
%  }
%  \subfloat[]{
%    \includegraphics[width=0.175\columnwidth]{images/tarantula/tarantula-310}
%    %\label{fig:mnist1-d}
%  }
%\caption{Tarantula with only one adversarial spectrum:
%(a) the original test input and the DNN predicts 'horse'
%(b) top 2\% ranked pixels by DeepCover for explaining the DNN's prediction
%(c) top 5\% ranked pixels
%and (d) top 10\% pixels}
%\label{fig:tarantula}
%\end{figure}

%\subsection{Target adversarial generation}

%\begin{table}[h!]
%  \begin{center}
%    \caption{Number of changed pixels for target adversarial geneeration: average number and standard derivation}
%    \label{tab:table1}
%    \begin{tabular}{c|c} % <-- Alignments: 1st column left, 2nd middle and 3rd right, with vertical lines in between
%      DeepCover & random \\
%      \hline
%      108 (132) & 149 (155)\\
%    \end{tabular}
%  \end{center}
%\end{table}


\subsection{Comparison with other tools}
In this part, we compare DeepCover with SHAP\footnote{https://github.com/slundberg/shap}~\cite{shap} and LIME\footnote{https://github.com/marcotcr/lime}~\cite{lime}, which are
the state-of-the-art techniques to analyse outputs from machine learning algorithms.
Particularly, we apply them on a set of traffic related ImageNet data. Examples are shown
in Figure \ref{fig:imagenet-data}

\begin{figure*}[!htb]
  \centering
  \subfloat[traffic light 1]{
    \includegraphics[width=0.2\linewidth]{images/imagenet-data/traffic_light1}
  }\hspace{0.cm}
  \subfloat[traffic light 2]{
    \includegraphics[width=0.2\linewidth]{images/imagenet-data/traffic_light2}
  }\hspace{0.cm}
  \subfloat[fire engine 1]{
    \includegraphics[width=0.2\linewidth]{images/imagenet-data/fireengine1}
  }\hspace{0.cm}
  \subfloat[fire engine 2]{
    \includegraphics[width=0.2\linewidth]{images/imagenet-data/fireengine2}
  }\hspace{0.cm}
  \caption{Examples of traffic related ImageNet inputs}
  \label{fig:imagenet-data}
\end{figure*}

\begin{figure*}[!htb]
  \centering
  \subfloat[]{
    \includegraphics[width=0.15\linewidth]{images/imagenet-example2/zoltar-1515}
  }\hspace{0.cm}
  \subfloat[]{
    \includegraphics[width=0.15\linewidth]{images/imagenet-example2/zoltar-3020}
  }\hspace{0.cm}
  \subfloat[]{
    \includegraphics[width=0.15\linewidth]{images/imagenet-example2/zoltar-7535}
  }\hspace{0.cm}
  \subfloat[]{
    \includegraphics[width=0.15\linewidth]{images/imagenet-example2/zoltar-15060}
  }
  \subfloat[]{
    \includegraphics[width=0.15\linewidth]{images/imagenet-example2/zoltar-30110}
  }\\  
  \subfloat[]{
    \includegraphics[width=0.15\linewidth]{images/imagenet-example3/zoltar-1515}
  }\hspace{0.cm}
  \subfloat[]{
    \includegraphics[width=0.15\linewidth]{images/imagenet-example3/zoltar-3020}
  }\hspace{0.cm}
  \subfloat[]{
    \includegraphics[width=0.15\linewidth]{images/imagenet-example3/zoltar-7535}
  }\hspace{0.cm}
  \subfloat[]{
    \includegraphics[width=0.15\linewidth]{images/imagenet-example3/zoltar-15060}
  }
  \subfloat[]{
    \includegraphics[width=0.15\linewidth]{images/imagenet-example3/zoltar-30110}
  }\\
  \subfloat[]{
    \includegraphics[width=0.15\linewidth]{images/imagenet-example4/zoltar-1515}
  }\hspace{0.cm}
  \subfloat[]{
    \includegraphics[width=0.15\linewidth]{images/imagenet-example4/zoltar-3020}
  }\hspace{0.cm}
  \subfloat[]{
    \includegraphics[width=0.15\linewidth]{images/imagenet-example4/zoltar-7535}
  }\hspace{0.cm}
  \subfloat[]{
    \includegraphics[width=0.15\linewidth]{images/imagenet-example4/zoltar-15060}
  }
  \subfloat[]{
    \includegraphics[width=0.15\linewidth]{images/imagenet-example4/zoltar-30110}
  }\\
  \subfloat[]{
    \includegraphics[width=0.15\linewidth]{images/imagenet-example5/zoltar-1515}
  }\hspace{0.cm}
  \subfloat[]{
    \includegraphics[width=0.15\linewidth]{images/imagenet-example5/zoltar-3020}
  }\hspace{0.cm}
  \subfloat[]{
    \includegraphics[width=0.15\linewidth]{images/imagenet-example5/zoltar-7535}
  }\hspace{0.cm}
  \subfloat[]{
    \includegraphics[width=0.15\linewidth]{images/imagenet-example5/zoltar-15060}
  }
  \subfloat[]{
    \includegraphics[width=0.15\linewidth]{images/imagenet-example5/zoltar-30110}
  }\\
  \caption{Explanations by DeepCover, with $\gamma\in\{1\%, 2\%, 5\%, 10\%, 20\%\}$, for the traffic related inputs in Figure \ref{fig:imagenet-data}}
  \label{fig:comp-deepcover}
\end{figure*}

\begin{figure*}[!htb]
  \centering
  \subfloat[traffic light 1]{
    \includegraphics[width=0.2\linewidth]{images/shap/traffic_light1}
  }\hspace{0.cm}
  \subfloat[traffic light 2]{
    \includegraphics[width=0.2\linewidth]{images/shap/traffic_light2}
  }\hspace{0.cm}
  \subfloat[fire engine 1]{
    \includegraphics[width=0.2\linewidth]{images/shap/fireengine1}
  }\hspace{0.cm}
  \subfloat[fire engine 2]{
    \includegraphics[width=0.2\linewidth]{images/shap/fireengine2}
  }\hspace{0.cm}
  \caption{Explanations by SHAP for the traffic related inputs in Figure \ref{fig:imagenet-data}: red pixels represent positive SHAP values that increase the probability of the class, while blue pixels reduce this probability}
  \label{fig:comp-shap}
\end{figure*}

\begin{figure*}[!htb]
  \centering
  \subfloat[]{
    \includegraphics[width=0.15\linewidth]{images/lime/lime1-5-features.png}
  }\hspace{0.cm}
  \subfloat[]{
    \includegraphics[width=0.15\linewidth]{images/lime/lime1-10-features.png}
  }\hspace{0.cm}
  \subfloat[]{
    \includegraphics[width=0.15\linewidth]{images/lime/lime1-20-features.png}
  }\hspace{0.cm}
  \subfloat[]{
    \includegraphics[width=0.15\linewidth]{images/lime/lime1-50-features.png}
  }
  \subfloat[]{
    \includegraphics[width=0.15\linewidth]{images/lime/lime1-500-features.png}
  }\\  
   \subfloat[]{
    \includegraphics[width=0.15\linewidth]{images/lime/lime2-5-features.png}
  }\hspace{0.cm}
  \subfloat[]{
    \includegraphics[width=0.15\linewidth]{images/lime/lime2-10-features.png}
  }\hspace{0.cm}
  \subfloat[]{
    \includegraphics[width=0.15\linewidth]{images/lime/lime2-20-features.png}
  }\hspace{0.cm}
  \subfloat[]{
    \includegraphics[width=0.15\linewidth]{images/lime/lime2-50-features.png}
  }
  \subfloat[]{
    \includegraphics[width=0.15\linewidth]{images/lime/lime2-500-features.png}
  }\\  
   \subfloat[]{
    \includegraphics[width=0.15\linewidth]{images/lime/lime3-5-features.png}
  }\hspace{0.cm}
  \subfloat[]{
    \includegraphics[width=0.15\linewidth]{images/lime/lime3-10-features.png}
  }\hspace{0.cm}
  \subfloat[]{
    \includegraphics[width=0.15\linewidth]{images/lime/lime3-20-features.png}
  }\hspace{0.cm}
  \subfloat[]{
    \includegraphics[width=0.15\linewidth]{images/lime/lime3-50-features.png}
  }
  \subfloat[]{
    \includegraphics[width=0.15\linewidth]{images/lime/lime3-500-features.png}
  }\\  
   \subfloat[]{
    \includegraphics[width=0.15\linewidth]{images/lime/lime4-5-features.png}
  }\hspace{0.cm}
  \subfloat[]{
    \includegraphics[width=0.15\linewidth]{images/lime/lime4-10-features.png}
  }\hspace{0.cm}
  \subfloat[]{
    \includegraphics[width=0.15\linewidth]{images/lime/lime4-20-features.png}
  }\hspace{0.cm}
  \subfloat[]{
    \includegraphics[width=0.15\linewidth]{images/lime/lime4-10-features.png}
  }
  \subfloat[]{
    \includegraphics[width=0.15\linewidth]{images/lime/lime4-500-features.png}
  }\\
  \caption{Explanations by LIME with different numbers, including 5, 10, 20, 50, 500, of top features for the traffic related inputs in Figure \ref{fig:imagenet-data}}
  \label{fig:comp-lime}
\end{figure*}

%LIME\cite{lime} is the state-of-the-art technique for understanding how 
%machine learning models make the decision. Besides the fundamental 
%theoretical difference between LIME and DeepCover, in this part we demonstrate
%by examples how they work differently.
%Figure \ref{fig:traffic-light} is the original traffic light image.
%Figure \ref{fig:lime} clearly exhibits how LIME and DeepCover explain the
%traffic light detection differently. 

%\begin{figure}[!htb]
%  \centering
%  \subfloat[]{
%    \includegraphics[width=0.5\linewidth]{images/lime-example1/origin}
%  }\hspace{0.cm}
%  \caption{Test inputs on traffic light detection}
%  \label{fig:traffic-light}
%\end{figure}

%\begin{figure*}[!htb]
%  \centering
%  \subfloat[]{
%    \includegraphics[width=0.225\linewidth]{images/lime-example1/5-features}
%  }\hspace{0.cm}
%  \subfloat[]{
%    \includegraphics[width=0.225\linewidth]{images/lime-example1/10-features}
%  }\hspace{0.cm}
%  \subfloat[]{
%    \includegraphics[width=0.225\linewidth]{images/lime-example1/20-features}
%  }\\
%  \subfloat[]{
%    \includegraphics[width=0.225\linewidth]{images/lime-example1/zoltar-3020}
%  }\hspace{0.cm}
%  \subfloat[]{
%    \includegraphics[width=0.225\linewidth]{images/lime-example1/zoltar-7535}
%  }\hspace{0.cm}
%  \subfloat[]{
%    \includegraphics[width=0.225\linewidth]{images/lime-example1/zoltar-15060}
%  }
%  \caption{Explanations on the traffic light detections from LIME and DeepCover}
%  \label{fig:lime}
%\end{figure*}


==> explain-model.tex <==
\section{Disjunctive Feature Attribution Model}
\label{sec:model}

A common explanation model, notably adopted by works like LIME~\cite{lime} and SHAP~\cite{shap},
is the additive feature attribution model. An additive explanation model is a linear function 
of binary variables such that
\begin{equation}
    \label{eq:additive}
    g(z')=\phi_0 + \sum_{i=1}^{M}\phi_i z_i'
\end{equation}
where $z'\in\{0,1\}^M$, $M$ is the number of simplified input feature and $\phi_i$ is the $i$th
simplified feature.

%As an example, in LIME, given an original input $x\in\mathbb{R}^{D_{L_0}}$, a binary vector
%$x'\in\{0,1\}^M$ is used to represent the "presence" and "absence" of each interpretable feature.

\paragraph{Limitations on the additive model}

The additive explanation model exhibits a simplified relationship between the model to be explained and
the interpretation. In fact, e have to admit that no interpretation model can perfectly represent the original model.
As a result, there most likely exists a complementary relationship between different interpretation models.
In the following, we take into account the disjunctive relationship between different interpretation models
for explaining a complex model.

We generalise the additive explanation model in \eqref{eq:additive} into a disjunctive manner.

\begin{definition}[Disjunctive Feature Attribute Model]
\label{def:disjunctive}
A disjunctive explanation model is a disjunctive formulation of multiple linear functions in the form of
\begin{equation}
    \label{eq:disjunctive}
    g(z')=\bigvee_k \varepsilon_k
\end{equation}
s.t. $\varepsilon_k=\phi_{k,0} + \sum_{i=1}^{M}\phi_{k,i} z_i'$.
\end{definition}

Disjunctive explanation is more generic and more expensive to achieve.
Non-surprisingly, works like SHAP and LIME cannot be applied to solve a disjunctive model.
In \cite{chu2018exact}, a closed form linear programming (LP) formulation is constructed, given an input
instance of a piecewise linear neural network; it can be expected that multiple such LP formulations 
indeed results in our disjunctive form.

Anyway, we are not going to solve a disjunctive explanation model. Instead, even when a disjunctive model is
assumed, our SBFL approach can be applied to localise important features in the input for the DNN decision.


==> related.tex <==
\section{Related Work}
\label{sec:related}

Youcheng: To re-write

\commentout{

This work connects two seemingly distinct research topics: spectrum-based fault localization and explainable AI.
We briefly summarize related research from software engineering and machine learning.

\paragraph*{Machine learning}
%community}

Explanation or interpretation of deep learning is a very active area in machine learning. Explanations of trained models is done by visualising hidden neurons, ranking input dimensions and other methods. LIME~\cite{lime} interprets model predictions by locally approximating the model around a given prediction. Based on LIME and a few other methods~\cite{STY2017, LRP, SGK2017, CAM}, SHAP~\cite{SHAP} suggests a general additive model and defines the importance value of each pixel as its Shapley value in a multi-player cooperative game, where each player represents a pixel. SHAP is the most up-to-date ranking method, and is compared with our method in the paper. The core of our proposed SBE method is also pixel ranking, however, our ranking uses the suspiciousness score computed by SBFL measures.
%\cite{chu2018exact}...

\paragraph*{Fault localization}
Our SBE approach is closely related to fault localization.
Besides the spectrum-based fault localization~\cite{naish2011model, lo2010comprehensive, lucia2014extended, wong2010family, zhang2017theoretical, perez2017test, jiang2011practical, santelices2009lightweight, feldt2016test, wong2016survey, zoltar, ochiai1957zoogeographic, jones2005empirical, wong2007effective,landsberg2015evaluation} discussed earlier in this paper, there are a large number of further fault localization methods, e.g.,
model based~\cite{birch2017fast, alves2017method}, slice based~\cite{Alves:2011}, interaction driven~\cite{li2016iterative,hao2009interactive},
similarity aware~\cite{hao2008similarity}, semantic fault localization~\cite{christakis2019semantic} and a number of others~\cite{kochhar2016practitioners, xia2016automated, zhou2012should, wong2014boosting}.
As indicated in work like~\cite{zou2019empirical, lucia2014fusion, wang2014version, le2015information}, there may be merit in combining different fault localization methods.
Meanwhile, work like~\cite{hao2010test, landsberg2018optimising, campos2013entropy, christi2018reduce} focus on better constructing
or optimizing the test suite for fault localization. Fault localization is related to automating fixes for programs~\cite{bohme2017bug, liu2019you}.
Genetic programming can be used to improve SBFL~\cite{Sohn2017xq,Choi2018aa}.

\paragraph*{Software engineering for AI}

There is a broad body of work on applying software engineering research to deep learning, and this paper is aligned with this idea. Among them, DeepFault~\cite{deepfault} is closest to ours. It applies spectrum-based fault localization to identify suspicious neurons that are responsible for inadequate DNN results; it is a white-box method and it was only tested on small benchmarks such as MNIST~\cite{MNIST} and CIFAR-10~\cite{krizhevsky2009learning}.
In~\cite{gopinath2018symbolic}, symbolic execution is used to find important pixels for the MNIST data set.

In~\cite{PCYJ2017,ma2018deepgauge, sun2018testing}, multiple structural test coverage criteria have been proposed for DNNs with the goal to support testing. The growing safety concern in deep learning based autonomous systems drives the work on testing methods for the DNN component~\cite{tian2017deeptest, deeproad, lan2018design}.  A number of testing approaches have been adopted for testing DNN models~\cite{ma2018combinatorial, deepmutation, sun2018concolic, udeshi2018automated, wang2018detecting, wang2018adversarial, kim2018guiding}. The most popular library to implement DNNs is TensorFlow~\cite{tensorflow} and an empirical study of TensorFlow program bugs can be found in~\cite{xiong-issta18}. 
}
%taint analysis  -- Youcheng to talk to John Galea


==> test-gen.tex <==
\section{Automated Test Case Generation}
\label{sec:test-gen}

\newcommand{\constraints}{\mathcal{C}}

We conjecture that the criteria proposed above achieve a good balance
between their ability to guide test case generation towards relevant cases
and their computational cost. To show this hypothesis, we now give two
algorithms for test case generation.

The test conditions required by our criteria exhibit particular combinations
between the condition features and the decision feature, and it is not
trivial to generate test cases for them.  Our methods for test case
generation are based on an observation made in the original version of this
paper~\cite{SHK2018}, and later confirmed in~\cite{odena2018tensorfuzz},
its approach to random test case generation is prohibitively inefficient for DNNs.  In
this section, we present two test generation algorithms: the first one is
based on linear programming (LP) and suitable for small to medium-sized DNNs
and the other based on gradient descent (GD), which scales to large
DNNs.
%
%We introduce for each test requirement $\requirements f$ for $f \in F$ an
%automatic test case generation algorithm
%$\textbf{Test-Gen}(\networks,\requirements f)$ to compute $\testsuites f$. 
%As we will explain later in Section~\ref{sec:random}, the generation of test
%suites for the criteria is non-trivial: a random testing approach will not
%achieve a test suite with high adequacy.  In this paper, we consider
%approaches based on constraint solving.  The algorithms are based on Linear
%Programming (LP).  
%
We~remark that, as is common in conventional software testing, our test
coverage criteria are not tied to any particular test case generation
algorithm, and thus, there exist alternative algorithms for generating test
suites that satisfy our criteria.

\subsection{Test Oracle}\label{sec:safety}

We clarify the usage of an oracle, which follows the idea of metamorphic
testing to determine \emph{automatically} whether a given test case $x$
has identified a bug in the DNN.
%
The DNN $\networks$ represents a function $\hat{\mathcal{F}}(x)$, which
approximates $\mathcal{F}(x): D_{L_1} \to \labels$ that models perfect human
perception capability.  Therefore, the ultimate safety requirement is that
for all test cases $x\in D_{L_1}$, we have $\hat{\mathcal{F}}(x) =
\mathcal{F}(x)$.  However, such a requirement is not practical because the
large number of inputs in $D_{L_1}$ and the high cost of asking humans to
label images.
%
A pragmatic compromise, as done in many other works
including~\cite{SZSBEGF2014, HKWW2017}, is to use the following
oracle as a proxy.

\begin{definition}[Oracle]
\label{def:requirement}
%
Given a finite set $X$ of correctly labeled inputs, an input $x'$ passes the
oracle if there exists some $x\in X$ such that $x$ and $x'$ are close
and $\hat{\mathcal{F}}(x') =
\hat{\mathcal{F}}(x)$.
%
\end{definition}

Ideally, the question of whether two inputs $x$ and $x'$ are close is to be
answered using human perception.  In practice, this is approximated by
various approaches, including norm-based distance measures.
%
%In this paper, the closeness of two inputs $x_1$ and $x_2$  is concretised as the norm $L^\infty$, i.e., $\distance{x_1-x_2}{\infty} \leq b$ for some bound $b \in \real$. 
%
Specifically, given the norm $L^p$ and an upper bound $b$ for the distance,
we say that two inputs $x$ and $x'$ are close iff $\distance{x-x'}{p} \leq
b$. We write $\mathit{close}(x,x')$ for this relation.
%
A pair of inputs that satisfies this definition are called
\emph{adversarial examples} if the label assigned to them by the
DNN differs.

The choice of $b$ is problem-specific.  In our experiments, we evaluate the
distribution of adversarial examples with respect to the distance (as
illustrated in Figure~\ref{fig:ss-distance-map} for one of the criteria). 
The use of this oracle constrains our approaches to regions of the input
domain that are close to one of the samples in the training dataset. 
Additional techniques may be required to qualify the DNN behaviour for other
parts of the input space.
%
%We remark that our algorithms can work with any definition of closeness as long as it can be encoded as a set of linear constraints. The test generation algorithms in this paper enable the computation of $x_1$ and $x_2$ such that $\distance{x_1-x_2}{\infty}$ 
%can be upper bounded by a small number.

%In our experiments, to exhibit the behavior of adversarial examples, 
%we instantiate $b$ with a large enough number, and study the percentage of adversarial examples with respect to the number $b$ (as illustrated in Figure~\ref{fig:ss-distance-map} for one of the criteria). 

\subsection{Test Case Generation with LP}
\label{sec:lp}

%The human perception function $\mathcal{F}$ represented by a DNN is
%highly non-linear and cannot be encoded with linear programming (LP)
%in general.  Therefore, other constraint solvers such as SMT
%\cite{HKWW2017,katz2017reluplex,bunel2017piecewise}, MILP
%\cite{LM2017,CNR2017,bunel2017piecewise,xiang2017output}, SAT
%\cite{NKPSW2017} have been considered.  However, it is computationally hard,
%if not impossible, for such direct encoding to handle large
%DNNs, because their underlying constraint solving problems are
%intractable (at least NP-hard).  
%
In this paper, for the efficient generation of a test case $x'$, we consider
(1)~an LP-based approach by fixing the a particular pattern of nodes'
activations according to a given input $x$, and (2)~encoding a prefix of the
network, instead of the entire network, with respect to a given feature
pair.

\begin{definition}[Activation Pattern]
%
Given 
%a network 
$\networks$ and 
%an input 
$x$, the activation pattern of
$\networks[x]$ is a function $ap[\networks,x]$, mapping from 
%the %set of
hidden nodes to the signs $\{+1,-1\}$, such that $ap[\networks,x](n_{k,i})=\mathit{sign}(n_{k,i},x)$ for $2\leq k<K$ and $1\leq i\leq s_k$.  
%
\end{definition}

%For an activation pattern $ap[x]$, 
For brevity, we may write $ap[\networks,x]$ as
$ap[x]$ if $\networks$ is clear from the context, and  write $ap[x]_{k,i}$ for $ap[\networks,x](n_{k,i})$. %to denote the sign
%of the $i$-th neuron at layer $k$. 

\begin{example}  (Continuation of Example~\ref{example:weights})
%
For input $x=(0,-1)$, by the activation values in
Table~\ref{tab:value-table}, we have $ap[x]_{2,1}=-1$, $ap[x]_{2,2}=+1$,
$ap[x]_{2,3}=-1$. 
%
\end{example}

In the following, we explain the LP encoding of a DNN instance,
$\networks[x]$ (Section~\ref{sec:encoding}), %introduce a few operations on
%the given activation pattern (Section~\ref{sec:operations}), discuss a
%safety requirement (Section~\ref{sec:safety}), 
and then present its use in the test case generation algorithm (Section \ref{sec:algorithms}).

\subsubsection{LP Model of a DNN Instance}\label{sec:encoding}

The variables used in the LP model are distinguished in \textbf{bold}.  All
variables are real-valued.  Given an input $x$, the input variable $\mathbf{x}$,
whose value is to be synthesized with LP, is required to have the identical
activation pattern as $x$, i.e., $ap[\mathbf{x}]=ap[x]$.


We use variables $\mathbf{u_{k,i}}$ and $\mathbf{v_{k,i}}$ to denote the valuations
of a node $n_{k,i}$ before and after the application of ReLU, respectively.
Then, we have the following set $\constraints_1[x]$ of constraints to encode
ReLU operations in a network instance.
%
\begin{equation}
\label{eq:lp-dir1}
\scalemath{0.9}{
\begin{array}{l}
 \{\mathbf{u_{k,i}}\geq 0 \wedge \mathbf{v_{k,i}}=\mathbf{u_{k,i}} ~|~ ap[x]_{k,i}\geq 0, k\in [2,K), i\in [1\dots s_k] \} \\
\cup 
  \{\mathbf{u_{k,i}}< 0 \wedge \mathbf{v_{k,i}}=0~|~ap[x]_{k,i}<0, k\in [2,K), i\in [1\dots s_k]\}
\end{array}
}
\end{equation}

Moreover, the activation valuation $\mathbf{u}_{k,i}$ of each node is
determined by the activation values $\mathbf{v}_{k-1,j}$ of those nodes in
the prior layer. This is defined as in Equation \eqref{eq:sum}. Therefore,
we add as the following set of constraints  $\constraints_2[x]$
for a symbolic encoding of nodes' activation values.
\begin{equation} \label{eq:lp-v}
\scalemath{0.85}{
\{  \mathbf{u}_{k,i}=\sum_{1\leq j \leq s_{k-1}} \{{w}_{k-1, j, i}\cdot \mathbf{v}_{k-1,j}\} + b_{k,i} ~|~ k\in [2,K), i\in [1\dots s_k]\}
}
\end{equation}
Please note that the resulting LP model $\constraints[x] =
\constraints_1[x]\cup \constraints_2[x]$  represents \emph{a symbolic set of
inputs} that have the identical activation pattern as $x$.
Further, we can specify some optimization objective $obj$, and call an LP solver
to find the optimal $\textbf{x}$ (if one exists). 

%\subsubsection{Operations on activation patterns}\label{sec:operations}

For simplicity, given the set $\constraints[x]$ (or simply $\constraints$) of constraints,
we  let $\constraints[x][1\dots k']$ be a partial encoding of
$\constraints[x]$ up to layer $k'$. More precisely, we write
$\constraints[x][1\dots k']$ if we substitute $K$ in Expression
(\ref{eq:lp-dir1}) and (\ref{eq:lp-v}) by $k'$. 
We also write $\constraints[x][1\dots k'(,i')]$ to denote that at layer $k'$ only the feature $\feature_{k',i'}$'s  activation needs to be encoded. Intuitively, the operation $[1\dots k'(,i')]$ is to have a partial encoding of Expression (\ref{eq:lp-dir1}) and (\ref{eq:lp-v}) focusing on a prefix of the network up to layer $k'-1$ with an additional feature $\feature_{k',i'}$ at layer $k'$. 

Note that, for every feature $\feature_{k,i}$, each its node in Expression~(\ref{eq:lp-dir1}) has either $\mathbf{u}\geq 0 \wedge \mathbf{v}=\mathbf{u}$ or $\mathbf{u}< 0 \wedge
\mathbf{v}=0$, but not both.  We write $\constraints[x](k,i)$
%and  $\constraints[x](k,i)_{-1}$
to denote the same  set  of constraints as $\constraints[x]$, except for  the sign change of the feature $\feature_{k,i}$. 

Assume that the value function $\valuefunction$ is linearly encodable.  
Without loss of generality, we still use $\valuefunction$  to denote its linear
encodings. We let $\constraints[+\valuefunction]= \constraints\cup \{\valuefunction\}$.




%We define a few operations on the set $\constraints[x]$, or simply $\constraints$, of constraints. 

%First, let $\constraints[x][1\dots k']$ be a partial encoding of
%$\constraints[x]$ up to layer $k'$. More precisely, we write
%$\constraints[x][1\dots k']$ if we substitute $K$ in Expression
%(\ref{eq:lp-dir1}) and (\ref{eq:lp-v}) by $k'$. 

%\begin{definition}\label{def:ap-partial}
%Let
%$\constraints[x][1\dots k']$ be a partial encoding of $\constraints[x]$ up to layer %$k'$. More precisely, we write $\constraints[x][1\dots k']$ if we substitute $K$ in %Expression (\ref{eq:lp-dir1}) and (\ref{eq:lp-v}) by $k'$. 
%\end{definition}

%For simplicity, we also write $\constraints[x][1\dots k'(,i')]$ to denote that at layer $k'$ only the neuron $n_{k',i'}$'s activation needs to be encoded. Intuitively, the operation $[1\dots k'(,i')]$ is to have a partial encoding of Expression (\ref{eq:lp-dir1}) and (\ref{eq:lp-v}) focusing on a prefix of the network up to layer $k'-1$ with an additional neuron $n_{k',i'}$ at layer $k'$. 
%
%that keeps identical activation signs for neurons until layer $k$. 
%That is, 
%However, for 
%For neurons beyond
%layer $k$, there are no constraints on $ap[x][:k]$. 
% does not require or specify their signs. 


%\paragraph{Actiavtion pattern with constraint set}

%Note that, for each neuron $n_{k,i}$, in Expression~(\ref{eq:lp-dir1}), we
%\mathbf{v}_{k,i}=\mathbf{u}_{k,i}$ or $\mathbf{u_{k,i}}< 0 \wedge
%\mathbf{v}_{k,i}=0$, but not both.  We write $\constraints_1[x](k,i)$ to
%denote the expression that is taken, and write $\constraints_1[x](k,i)_{-1}$
%to denote the other expression that is not taken.

%\begin{definition}\label{def:ap-except}
%
%  Let $\constraints[x][(k,i)]$ be the same set of constraints as $\constraints[x]$,
%except that the constraint  $\constraints_1[x](k,i)$ is substituted by
%$\constraints_1[x](k,i)_{-1}$.
%
%end{definition}

%Assume that the value function $\valuefunction$ and the distance function
%$\distancefunction$ are linearly encodable.  Without loss of generality, we
%still use $\valuefunction$ and $\distancefunction$ to denote their linear
%encodings, respectively.

%\begin{definition}
%Let $\constraints[+\valuefunction]= \constraints\cup \{\valuefunction\}$ and %$\constraints[+\distancefunction]=\constraints\cup \{\distancefunction \}$.  
%\end{definition}
%
%Let $lb_{k,i}, ub_{k,i} \in \real$ be the real numbers such that $lb_{k,i} \leq ub_{k,i}$. Now, we define $C[\alpha]$ for $\alpha \subseteq \Omega$ where 
%\begin{equation}
%\Omega= \{(k,i), \mathbf{u_{k,i}} \in [lb_{k,i}, ub_{k,i}]~|~ k\in (2,K], i\in [1..s_k]\}\end{equation} 
%
%
%For example, when requiring a neuron $n_{k,i}$ to be activated with values
%bounded by $[lb_{k,i}, ub_{k,i}]$, we can use the following operation
%$\constraints[+ (\mathbf{u_{k,i}} \in [lb_{k,i}, ub_{k,i}])]$.

Furthermore, we can generalize the above notation and define
$\constraints[ops]$ for $ops$ 
%being 
a set of operations.  It is obvious that
the ordering of the operations does not matter if there does not exist a
feature whose value is affected by more than one operation in $ops$.

\subsubsection{Automatic Test Generation Algorithms}\label{sec:algorithms}

Our test criteria, defined in Section~\ref{sec:criteria}, identify that the
(sign or value) change of every decision feature must be supported by (sign
or value) changes of its condition features.  Given a feature pair
and a test criterion, we are going to find two activation patterns, and
the two patterns together shall exhibit the changes required by the
corresponding test criterion.  The inputs matching these patterns
will be added to the final test suite.

We use a routine $lp\_call$ to call the LP solver. The routine takes as input a
set $\constraints$ of constraints and an optimization objective $obj$,
and returns a valuation $x$ for input variable $\textbf{x}$ if one exists. 
%For instance, a solver call can be written  as follows.
%
%\begin{equation}
%  \label{eq:lp-call}
% x = lp\_call(\constraints, obj)
%\end{equation}
%
%It returns an input $\textbf{x}$ (if there exists), which 
%If returned successfully, $x$ satisfies the linear constraints of $\constraints$, with respect to
%the optimization objective $obj$.
%
%\paragraph{Test suite generation}
%
The test suite generation framework is given  in Algorithm
\ref{algo:test-gen}: for every $(\feature_{k,i},\feature_{k+1,j})$ of
$O$, it calls the $get\_input\_pair(f,\feature_{k,i},\feature_{k+1,j})$
method to find an input pair that satisfies the test condition, according
to the covering method $f\in
\{\covered{SS}{}{},\covered{VS}{\valuefunction}{},\covered{SV}{\valuefunction}{},$ $\covered{VV}{\valuefunction,\valuefunction}{}\}$.
Recall that $O\subseteq \neuronpairs(\networks)$ is a set of feature pairs of a DNN.
%(see Definition~\ref{def:neuron-pair}).


\begin{algorithm}[!htp]
  \caption{Test-Gen($\networks$, $f$)}\label{algo:test-gen}
  %\begin{flushleft}
  %  \textbf{INPUT:} DNN $\networks$, covering method $f$\\
  %  \textbf{OUTPUT:} test suite $\mathcal{T}$, adversarial examples $\mathcal{T}'$
  %\end{flushleft}
  \begin{algorithmic}[0] %[1]
    \For{each feature pair $\feature_{k,i}, \feature_{k+1,j}\in O$}
      \State $x_1,x_2=get\_input\_pair(f,\feature_{k,i}, \feature_{k+1,j})$
      \If{$x_1,x_2$ are valid inputs}
        \State $\mathcal{T}\leftarrow\mathcal{T}\cup\{x_1, x_2\}$
        \If{$\networks[x_1].\mathit{label}\neq \networks[x_2].\mathit{label}$ and $close(x_1,x_2)$}
          \State $\mathcal{T}'\leftarrow\mathcal{T}'\cup\{x_1, x_2\}$
        \EndIf
      \EndIf
    \EndFor
    \State\Return{$\mathcal{T}, \mathcal{T}'$}
  \end{algorithmic}
\end{algorithm}


In the following, we instantiate the function $get\_input\_pair$. 
To get an input pair of tests for each corresponding feature pair
$(\feature_{k,i}, \feature_{k+1,j})$, we assume the existence of
a $data\_set$ of correctly labeled inputs.  An input $x_1$
in $data\_set$ serves for the reference activation pattern, by modifying
which we obtain another activation pattern such that the two together shall
be able to support testing conditions specified by the covering method for the
feature pair $\feature_{k,i}$ and $\feature_{k+1,j}$.

Algorithm \ref{algo:aac-get-input-pair} tries to find a pair of inputs that
 SS-cover the feature pair.
%, which specify that
%the sign change of $\feature_{k,i}$ must independently change also the sign of
%$\feature_{k+1,j}$.  
In particular, the LP call in
Algorithm~\ref{algo:aac-get-input-pair} comes with the constraints that a
new activation pattern must share the partial encoding of $x_1$'s activation
pattern until layer $k$ together with the feature $\feature_{k+1,j}$ 
(by imposing operation  $[1\dots k+1(,j)]$ on $\constraints[x_1]$
%, as defined in Definition~\ref{def:ap-partial}
), but with signs of features $\feature_{k,i}$ and 
$\feature_{k+1,j}$'s activation being negated (by imposing operation $[\{(k,i), (k+1,j)\}]$
on $\constraints[x_1][1\dots k+1(,j)]$. %, as defined in Definition \ref{def:ap-except}).  
As a matter of fact, this encoding is even
stronger than the definition for SS coverage, which does not
specify constraints for nodes in prior to layer $k$.  The encoding in the
$lp\_call$ is a compromise for efficiency, as it is computationally
un-affordable to consider combinations of even a subset of neuron
activations.  Consequently, the LP call may fail because the proposed
activation pattern is infeasible, and this explains why we need 
%to 
%prepare 
a
$data\_set$ for potentially multiple LP calls.

\begin{algorithm}[!htp]
  \caption{$get\_input\_pair(f, \feature_{k,i},\feature_{k+1,j})$ when $f=\covered{SS}{}{}$}
  \label{algo:aac-get-input-pair}
  %\begin{flushleft}
  %  \textbf{INPUT:} $\covered{SS}{}{}$, feature pair $\feature_{k,i},\feature_{k+1,j}$\\
  %  \textbf{OUTPUT:} input pair $x_1, x_2$
  %\end{flushleft}
  \begin{algorithmic}%[1]
    \For{each $x_1 \in data\_set$}
    %\State $\alpha=C[x_1]$
    \State $\scalemath{0.85}{x_2\leftarrow lp\_call(\constraints[x_1][1\dots k+1(,j)][\{(k,i), (k+1,j)\}], \min{\distance{x_2\!-\!x_1}{\infty}})}$
      \If{ $x_2$ is a valid input} \Return {$x_1,x_2$}

      \EndIf
    \EndFor
    \State \Return{None, None}
  \end{algorithmic}
\end{algorithm}

The functions that find input pairs subject to 
%the 
other covering methods
largely follow the same structure as the SS coverage case, with the addition
of value change constraints. % Note that when implementing
%test generation for $cov^{\valuefunction}_{VS}$ and $cov^{\valuefunction_1,\valuefunction_2}_{VV}$,
%there is no need to go through every feature pair, as these metrics do not require the
%individual change of a particular condition neuron as long as the overall
%behavior of all condition neurons of the decision neuron fall into certain
%distance change (and they do not exhibit sign change).
In particular, given an original input $x_1$, the linear constraints argument for $lp\_call$ 
are constructed as follows:
\begin{itemize}
    \item when $f=\covered{VS}{\valuefunction}{}$:
    $\constraints[x_1][1\dots k(,i)][\{(k,i),+\valuefunction\}]$
    \item when $f=\covered{SV}{\valuefunction}$: 
    $\constraints[x_1][1\dots k+1(,j)][\{(k,i), +\valuefunction\}]$
    \item when $f=\covered{VV}{\valuefunction_1,\valuefunction_2}{}$: 
    $\constraints[x_1][1\dots k,(i)][\{+\valuefunction_1, +\valuefunction_2\}]$
\end{itemize}

\commentout{

\begin{algorithm}[!htp]
  \caption{$get\_input\_pair$ with the first argument being $\covered{DS}{\distancefunction}{}$}
  \begin{flushleft}
    \textbf{INPUT:} $\covered{DS}{\distancefunction}{}$, neuron $n_{k,i}$\\
    \textbf{OUTPUT:} input pair $x_1, x_2$
  \end{flushleft}
  \begin{algorithmic}[1]
    \For{each $x_1 \in data\_set$}
    \State $x_2=lp\_call(\constraints[x_1][1\dots k(,i)][\{(k,i),+\distancefunction\}], \min{\distance{x_2\!-\!x_1}{\infty}})$
      \If{ $x_2$ is a valid input} \Return {$x_1,x_2$}
      \EndIf
    \EndFor
    \State \Return{\_, \_}
    \label{algo:ds-get-input-pair}
  \end{algorithmic}
\end{algorithm}

%Then, similar as in the SS case, by applying Algorithm \ref{algo:ds-get-input-pair} on each neuron, we are
%able to obtain a test suite that covers DS requirements, and a set of adversarial examples found during the
%test generation. 

%\paragraph{SV test suite generation}

\begin{algorithm}[!htp]
  \caption{$get\_input\_pair$ with the first argument being $\covered{SV}{\valuefunction}{}$}
  \begin{flushleft}
    \textbf{INPUT:} $\covered{SV}{\valuefunction}{}$, neuron pair $n_{k,i},n_{k+1,j}$\\
    \textbf{OUTPUT:} input pair $x_1, x_2$
  \end{flushleft}
  \begin{algorithmic}[1]
    \For{each $x_1 \in data\_set$}
    \State $x_2\!=\!lp\_call(\constraints[x_1][1\dots k+1(,j)][\{(k,i), +\valuefunction\}], \min{\distance{x_2\!-\!x_1}{\infty}})$
      \If{ $x_2$ is a valid input} \Return {$x_1,x_2$}
      \EndIf
    \EndFor
    \State \Return{\_, \_}
    \label{algo:sv-get-input-pair}
  \end{algorithmic}
\end{algorithm}

%\paragraph{DV test suite generation}

\begin{algorithm}[!htp]
  \caption{$get\_input\_pair$  with the first argument being $\covered{DV}{\distancefunction,\valuefunction}{}$}
  \begin{flushleft}
    \textbf{INPUT:} $\covered{DV}{\distancefunction,\valuefunction}{}$, neuron $n_{k,i}$\\
    \textbf{OUTPUT:} input pair $x_1, x_2$
  \end{flushleft}
  \begin{algorithmic}[1]
    \For{each $x_1 \in data\_set$}
    \State $x_2=lp\_call(\constraints[x_1][1\dots k,(i)][\{+\valuefunction, +\distancefunction\}], \min{\distance{x_2\!-\!x_1}{\infty}})$
      \If{ $x_2$ is a valid input} \Return {$x_1,x_2$}
      \EndIf
    \EndFor
    \State \Return{\_, \_}
    \label{algo:dv-get-input-pair}
  \end{algorithmic}
\end{algorithm}
}

In our implementation, every time the $get\_input\_pair$ is called we
randomly select 40 correctly labeled inputs to construct the $data\_set$. 
The objective $\min{\distance{x_2\!-\!x_1}{\infty}}$ is used in all LP
calls, to find good adversarial examples with respect to the safety
requirement.  Moreover, we use 
$\valuefunction = \frac{u_{k+1,j}[x_2]}{u_{k+1,j}[x_1]}\geq \sigma$
%
%\begin{equation}
%\valuefunction = \frac{u_{k+1,j}[x_2]}{u_{k+1,j}[x_1]}\geq \sigma
%\end{equation} 
%
with $\sigma=2$ for $g$ in $SV^g$ and $\sigma=5$ for
$VV^{\valuefunction_1, \valuefunction_2}$ (with respect to $\valuefunction_2$).  
We admit that such choices are experimental.  Meanwhile, for generality and to
speed up the experiments, we leave the value function $\valuefunction_1$ unspecified. 
Providing a specific $\valuefunction_1$ may require more LP calls to find a
$x_2$ (because $\valuefunction_1$ is an additional constraint) but the
resulting $x_2$ can be better.
%with respect to $\valuefunction_1$.





\commentout{
\subsection{$M\covered{SS}{}{}$ and $M\covered{SV}{\valuefunction}{}$ with Top Weights}


For the two criteria $M\covered{SS}{}{}$ and $M\covered{SV}{\valuefunction}{}$,  we need to call the function $get\_input\_pair$  
$|\neuronpairs(\networks)|$ times. 
We note that $|\neuronpairs(\networks)|= \sum_{k=2}^{K} s_k \cdot s_{k-1}$. 
Therefore, when the size of the network is large, the generation of a test
suite may take a  long time.  To work around this, we may consider an
alternative definition of $\neuronpairs(\networks)$ by letting
$(n_{k,i},n_{k+1,j})\in \neuronpairs(\networks)$ only when the weight
is one of the $\kappa$ largest among $\{|w_{k,i',j}|~|~i'\in
[1\dots s_{k}]\}$.  The rationale behind is that condition neurons do not
equally affect their decision, and those with higher (absolute) weights are
likely to have a larger influence.

}


\subsection{Test Case generation: a Heuristic Search }

The LP optimisation in Algorithm \ref{algo:aac-get-input-pair} has strong
guarantee that is able to return an input pair as long as one exists. However,
its scalability depends on the efficiency of LP solvers and it is not trivial to apply such
a testing method to large-scale DNNs with millions of neurons. In this part, instead we develop
a heuristic algorithm  based on the gradient search. Note that, following the gradient change has been widely shown efficient in finding bugs in DNNs and has been utilised in existing 
DNN testing methods (e.g., \cite{PCYJ2017,ma2018deepgauge,deepmutation}).

\begin{algorithm}[!htp]
  \caption{$get\_input\_pair(f, \feature_{k,i},\feature_{k+1,j})$}
%  (a heuristic)}

  \label{algo:aac-get-input-pair-search}
  \begin{algorithmic}%[1]
    \For{each $x_1 \in data\_set$}
      \State sample an input  $x_2$ and a positive number $\epsilon$ %s.t. $x_1$ and $x_2$ are far enough from each other
      \For{a bounded number of steps}
        %\If{$(x_1, x_2)\models f(\feature_{k,i},\feature_{k+1,j})$} \Return{$x_1,x_2$}  \EndIf
        %\If{$(x_1, x_2)\models^{>} req(f, \feature_{k,i},\feature_{k+1,j})$} $x_2\leftarrow x_2-\epsilon\cdot\nabla\hat{\mathcal{F}}(x_2)$
        \If{$f((\feature_{k,i},\feature_{k+1,j}),x_1, x_2)$} \Return{$x_1,x_2$}  \EndIf
        \State update $\epsilon$       
        %\If{$f(x_1, x_2)\not\models f(\feature_{k,i},\feature_{k+1,j})/\feature_{k,i},\feature_{k+1,j}$}
        \If{$\neg f^{widen}((\feature_{k,i},\feature_{k+1,j}),x_1, x_2)$} $x_2\leftarrow x_2-\epsilon\cdot\nabla\hat{\mathcal{F}}(x_2)$
        \Else {$\,\,\,x_2\leftarrow x_2+\epsilon\cdot\nabla\hat{\mathcal{F}}(x_2)$}
        \EndIf 
      \EndFor
    \EndFor
    \State \Return{None, None}
  \end{algorithmic}
\end{algorithm}
The algorithm, depicted in Algorithm \ref{algo:aac-get-input-pair-search}, is 
to find an input pair $x_1, x_2$ such that the test condition 
by the covering method $f$ on the feature pair $\neuronpair=(\feature_{k,i},\feature_{k+1,j})$
is satisfied, i.e., $f(\neuronpair, x_1, x_2)$ is $\true$.
We use $f^{widen}(\neuronpair, x_1, x_2)$ for a widened version
of the testing condition by $f$ such that all its predicates on the features $\feature_{k,i}$
and $\feature_{k+1,j}$ are eliminated. It is supposed that $x_1$ is given and intuitively, starting from  an input $x_2$, if the feature changes other than $\feature_{k,i}$ and 
$\feature_{k+1,j}$ do not meet requirements by $f$, $x_2$ is moved closer to $x_1$, by following
the gradient descent: $x_2\leftarrow x_2-\epsilon\cdot\nabla\hat{\mathcal{F}}(x_2)$, as an attempt to counteract such changes. This applies to the case when the activation sign changes on other condition features. Otherwise, the change between $x_1$ and $x_2$ can only exploit a subset of 
predicates (in the testing condition) from the given feature pair, and we update $x_2$
following the gradient ascent. The algorithm's gradient change follows an adaptive manner that
comprises of a local search to update $x_2$ at each step and a simple strategy for 
the overall search direction to move closer/further with respect to $x_1$. 
In our implementation, we apply  FGSM (Fast Gradient Sign Method) \cite{FGSM}
 to initialise $x_2$ and $\epsilon$, and then we use a binary search scheme to update 
$\epsilon$ at each step.
